LLM For Loop Invariant Generation and Fixing: How Far Are We?

A loop invariant is a property of a loop that remains true before and after each execution of the loop. The identification of loop invariants is a critical step to support automated program safety assessment. Recent advancements in Large Language Models (LLMs) have demonstrated potential in diverse software engineering (SE) and formal verification tasks. However, we are not aware of the performance of LLMs to infer loop invariants. We report an empirical study of both open-source and closed-source LLMs of varying sizes to assess their proficiency in inferring inductive loop invariants for programs and in fixing incorrect invariants. Our findings reveal that while LLMs exhibit some utility in inferring and repairing loop invariants, their performance is substantially enhanced when supplemented with auxiliary information such as domain knowledge and illustrative examples. LLMs achieve a maximum success rate of 78\% in generating, but are limited to 16\% in repairing the invariant.

==> bibitem.tex <==
\bibitem{gulwani2009constraint}Gulwani, S., Srivastava, S. \& Venkatesan, R. Constraint-based invariant inference over predicate abstraction. {\em Verification, Model Checking, And Abstract Interpretation: 10th International Conference, VMCAI 2009, Savannah, GA, USA, January 18-20, 2009. Proceedings 10}. pp. 120-135 (2009)
\bibitem{de2008z3}De Moura, L. \& Bjørner, N. Z3: An efficient SMT solver. {\em International Conference On Tools And Algorithms For The Construction And Analysis Of Systems}. pp. 337-340 (2008)
\bibitem{lahiri2007predicate}Lahiri, S. \& Bryant, R. Predicate abstraction with indexed predicates. {\em ACM Transactions On Computational Logic (TOCL)}. \textbf{9}, 4-es (2007)
\bibitem{karr1976affine}Karr, M. Affine relationships among variables of a program. {\em Acta Informatica}. \textbf{6}, 133-151 (1976)
\bibitem{barbosa2022cvc5}Barbosa, H., Barrett, C., Brain, M., Kremer, G., Lachnitt, H., Mann, M., Mohamed, A., Mohamed, M., Niemetz, A., Nötzli, A. \& Others cvc5: A versatile and industrial-strength SMT solver. {\em International Conference On Tools And Algorithms For The Construction And Analysis Of Systems}. pp. 415-442 (2022)
\bibitem{clarke2003counterexample}Clarke, E., Grumberg, O., Jha, S., Lu, Y. \& Veith, H. Counterexample-guided abstraction refinement for symbolic model checking. {\em Journal Of The ACM (JACM)}. \textbf{50}, 752-794 (2003)
\bibitem{mcmillan2010lazy}McMillan, K. Lazy annotation for program testing and verification. {\em Computer Aided Verification: 22nd International Conference, CAV 2010, Edinburgh, UK, July 15-19, 2010. Proceedings 22}. pp. 104-118 (2010)
\bibitem{dillig2013inductive}Dillig, I., Dillig, T., Li, B. \& McMillan, K. Inductive invariant generation via abductive inference. {\em Acm Sigplan Notices}. \textbf{48}, 443-456 (2013)
\bibitem{zhu2015learning}Zhu, H., Nori, A. \& Jagannathan, S. Learning refinement types. {\em ACM SIGPLAN Notices}. \textbf{50}, 400-411 (2015)
\bibitem{sharma2016invariant}Sharma, R. \& Aiken, A. From invariant checking to invariant inference using randomized search. {\em Formal Methods In System Design}. \textbf{48} pp. 235-256 (2016)
\bibitem{chakraborty2023ranking}Chakraborty, S., Lahiri, S., Fakhoury, S., Musuvathi, M., Lal, A., Rastogi, A., Senthilnathan, A., Sharma, R. \& Swamy, N. Ranking llm-generated loop invariants for program verification. {\em ArXiv Preprint ArXiv:2310.09342}. (2023)
\bibitem{furia2014loop}Furia, C., Meyer, B. \& Velder, S. Loop invariants: Analysis, classification, and examples. {\em ACM Computing Surveys (CSUR)}. \textbf{46}, 1-51 (2014)
\bibitem{padhi2016data}Padhi, S., Sharma, R. \& Millstein, T. Data-driven precondition inference with learned features. {\em ACM SIGPLAN Notices}. \textbf{51}, 42-56 (2016)
\bibitem{fedyukovich2018accelerating}Fedyukovich, G. \& Bodı́k, R. Accelerating syntax-guided invariant synthesis. {\em Tools And Algorithms For The Construction And Analysis Of Systems: 24th International Conference, TACAS 2018, Held As Part Of The European Joint Conferences On Theory And Practice Of Software, ETAPS 2018, Thessaloniki, Greece, April 14-20, 2018, Proceedings, Part I 24}. pp. 251-269 (2018)
\bibitem{flanagan2001houdini}Flanagan, C. \& Leino, K. Houdini, an annotation assistant for ESC/Java. {\em International Symposium Of Formal Methods Europe}. pp. 500-517 (2001)
\bibitem{garg2016learning}Garg, P., Neider, D., Madhusudan, P. \& Roth, D. Learning invariants using decision trees and implication counterexamples. {\em ACM Sigplan Notices}. \textbf{51}, 499-512 (2016)
\bibitem{li2017automatic}Li, J., Sun, J., Li, L., Le, Q. \& Lin, S. Automatic loop-invariant generation anc refinement through selective sampling. {\em 2017 32nd IEEE/ACM International Conference On Automated Software Engineering (ASE)}. pp. 782-792 (2017)
\bibitem{ezudheen2018horn}Ezudheen, P., Neider, D., D'Souza, D., Garg, P. \& Madhusudan, P. Horn-ICE learning for synthesizing invariants and contracts. {\em Proceedings Of The ACM On Programming Languages}. \textbf{2}, 1-25 (2018)
\bibitem{chu2024better}Chu, K., Chen, Y. \& Nakayama, H. A Better LLM Evaluator for Text Generation: The Impact of Prompt Output Sequencing and Optimization. {\em ArXiv Preprint ArXiv:2406.09972}. (2024)
\bibitem{jhala2006practical}Jhala, R. \& McMillan, K. A practical and complete approach to predicate refinement. {\em International Conference On Tools And Algorithms For The Construction And Analysis Of Systems}. pp. 459-473 (2006)
\bibitem{corr18padhi}Padhi, S., Sharma, R. \& Millstein, T. LoopInvGen: A Loop Invariant Generator based on Precondition Inference. {\em CoRR}. \textbf{abs/1707.02029} (2018), http://arxiv.org/abs/1707.02029
\bibitem{gupta2009tests}Gupta, A., Majumdar, R. \& Rybalchenko, A. From tests to proofs. {\em International Conference On Tools And Algorithms For The Construction And Analysis Of Systems}. pp. 262-276 (2009)
\bibitem{colon2003linear}Colón, M., Sankaranarayanan, S. \& Sipma, H. Linear invariant generation using non-linear constraint solving. {\em Computer Aided Verification: 15th International Conference, CAV 2003, Boulder, CO, USA, July 8-12, 2003. Proceedings 15}. pp. 420-432 (2003)
\bibitem{kamath2023finding}Kamath, A., Senthilnathan, A., Chakraborty, S., Deligiannis, P., Lahiri, S., Lal, A., Rastogi, A., Roy, S. \& Sharma, R. Finding inductive loop invariants using large language models. {\em ArXiv Preprint ArXiv:2311.07948}. (2023)
\bibitem{ernst2007daikon}Ernst, M., Perkins, J., Guo, P., McCamant, S., Pacheco, C., Tschantz, M. \& Xiao, C. The Daikon system for dynamic detection of likely invariants. {\em Science Of Computer Programming}. \textbf{69}, 35-45 (2007)
\bibitem{le2019sling}Le, T., Zheng, G. \& Nguyen, T. SLING: using dynamic analysis to infer program invariants in separation logic. {\em Proceedings Of The 40th ACM SIGPLAN Conference On Programming Language Design And Implementation}. pp. 788-801 (2019)
\bibitem{flanagan2002predicate}Flanagan, C. \& Qadeer, S. Predicate abstraction for software verification. {\em Proceedings Of The 29th ACM SIGPLAN-SIGACT Symposium On Principles Of Programming Languages}. pp. 191-202 (2002)
\bibitem{hoare1969axiomatic}Hoare, C. An axiomatic basis for computer programming. {\em Communications Of The ACM}. \textbf{12}, 576-580 (1969)
\bibitem{yao2020learning}Yao, J., Ryan, G., Wong, J., Jana, S. \& Gu, R. Learning nonlinear loop invariants with gated continuous logic networks. {\em Proceedings Of The 41st ACM SIGPLAN Conference On Programming Language Design And Implementation}. pp. 106-120 (2020)
\bibitem{barrett2011cvc4}Barrett, C., Conway, C., Deters, M., Hadarean, L., Jovanović, D., King, T., Reynolds, A. \& Tinelli, C. cvc4. {\em Computer Aided Verification: 23rd International Conference, CAV 2011, Snowbird, UT, USA, July 14-20, 2011. Proceedings 23}. pp. 171-177 (2011)
\bibitem{misu2024towards}Misu, M., Lopes, C., Ma, I. \& Noble, J. Towards ai-assisted synthesis of verified dafny methods. {\em Proceedings Of The ACM On Software Engineering}. \textbf{1}, 812-835 (2024)
\bibitem{achiam2023gpt}Achiam, J., Adler, S., Agarwal, S., Ahmad, L., Akkaya, I., Aleman, F., Almeida, D., Altenschmidt, J., Altman, S., Anadkat, S. \& Others Gpt-4 technical report. {\em ArXiv Preprint ArXiv:2303.08774}. (2023)
\bibitem{si2018learning}Si, X., Dai, H., Raghothaman, M., Naik, M. \& Song, L. Learning loop invariants for program verification. {\em Advances In Neural Information Processing Systems}. \textbf{31} (2018)
\bibitem{echenim2019ilinva}Echenim, M., Peltier, N. \& Sellami, Y. Ilinva: Using abduction to generate loop invariants. {\em Frontiers Of Combining Systems: 12th International Symposium, FroCoS 2019, London, UK, September 4-6, 2019, Proceedings 12}. pp. 77-93 (2019)
\bibitem{uddin2022empirical}Uddin, G., Guéhénuc, Y., Khomh, F. \& Roy, C. An empirical study of the effectiveness of an ensemble of stand-alone sentiment detection tools for software engineering datasets. {\em ACM Transactions On Software Engineering And Methodology (TOSEM)}. \textbf{31}, 1-38 (2022)
\bibitem{alur2013syntax}Alur, R., Bodik, R., Juniwal, G., Martin, M., Raghothaman, M., Seshia, S., Singh, R., Solar-Lezama, A., Torlak, E. \& Udupa, A. Syntax-guided synthesis. (IEEE,2013)

\bibitem{wu2024llm}Wu, G., Cao, W., Yao, Y., Wei, H., Chen, T. \& Ma, X. LLM Meets Bounded Model Checking: Neuro-symbolic Loop Invariant Inference. {\em Proceedings Of The 39th IEEE/ACM International Conference On Automated Software Engineering}. pp. 406-417 (2024)


\bibitem{pei2023can}
K. Pei, S. Wang, Z. Zhang, J. Yang, and S. Jana, “Can large language models reason about program invariants?,” in \textit{Int. Conf. on Machine Learning (ICML)}, pp. 27496–27520, PMLR, 2023.



\bibitem{wu2023lemur}
H. Wu, C. Barrett, and N. Narodytska, “Lemur: Integrating large language models in automated program verification,” \textit{arXiv preprint arXiv:2310.04870}, 2023.

\bibitem{mistral_large}
Mistral AI, “Mistral Large,” 2024. [Online]. Available: https://mistral.ai/models. [Accessed: Mar. 8, 2025].

\bibitem{meta2024llama3}
Meta AI, “Meta Llama 3.1,” 2024. [Online]. Available: https://ai.meta.com/blog/meta-llama-3-1/. [Accessed: Jul. 29, 2024].

\bibitem{si2020code2inv}
X. Si, A. Naik, H. Dai, M. Naik, and L. Song, “Code2inv: A deep learning framework for program verification,” in \textit{Proc. 32nd Int. Conf. on Computer Aided Verification (CAV)}, Los Angeles, CA, USA, Jul. 2020, pp. 151–164, Springer.

\bibitem{chen2021evaluating}
M. Chen, J. Tworek, H. Jun, Q. Yuan, H. P. de Oliveira Pinto, J. Kaplan, H. Edwards, Y. Burda, N. Joseph, G. Brockman, \textit{et al.}, “Evaluating large language models trained on code,” \textit{arXiv preprint arXiv:2107.03374}, 2021.

\bibitem{chowdhery2022palm}
A. Chowdhery, S. Narang, J. Devlin, M. Bosma, G. Mishra, A. Roberts, P. Barham, H. W. Chung, C. Sutton, S. Gehrmann, \textit{et al.}, “PaLM: Scaling language modeling with pathways,” \textit{arXiv preprint arXiv:2204.02311}, vol. 10, p. 1, 2022.

\bibitem{chang2024survey}
Y. Chang, X. Wang, J. Wang, Y. Wu, L. Yang, K. Zhu, H. Chen, X. Yi, C. Wang, Y. Wang, \textit{et al.}, “A survey on evaluation of large language models,” \textit{ACM Trans. Intell. Syst. Technol.}, vol. 15, no. 3, pp. 1–45, 2024.


\bibitem{hrushovski2023strongest}
E. Hrushovski, J. Ouaknine, A. Pouly, and J. Worrell,
"On strongest algebraic program invariants," 
\textit{Journal of the ACM}, vol. 70, no. 5, pp. 1--22, 2023.

\bibitem{muller2004computing}
M. Müller-Olm and H. Seidl,
"Computing polynomial program invariants," 
\textit{Information Processing Letters}, vol. 91, no. 5, pp. 233--244, 2004.

\bibitem{yu2023loop}
S. Yu, T. Wang, and J. Wang,
"Loop Invariant Inference through SMT Solving Enhanced Reinforcement Learning," 
in \textit{Proc. of the 32nd ACM SIGSOFT International Symposium on Software Testing and Analysis}, pp. 175--187, 2023.

\bibitem{si2018learning}
X. Si, H. Dai, M. Raghothaman, M. Naik, and L. Song,
"Learning loop invariants for program verification," 
\textit{Advances in Neural Information Processing Systems}, vol. 31, 2018.

\bibitem{pawlik2016tree}
M. Pawlik and N. Augsten,
"Tree edit distance: Robust and memory-efficient," 
\textit{Information Systems}, vol. 56, pp. 157--173, 2016.

\bibitem{pawlik2015efficient}
M. Pawlik and N. Augsten,
"Efficient computation of the tree edit distance," 
\textit{ACM Trans. Database Syst.}, vol. 40, no. 1, pp. 1--40, 2015.

\bibitem{pawlik2011rted}
M. Pawlik and N. Augsten,
"RTED: a robust algorithm for the tree edit distance," 
\textit{arXiv preprint arXiv:1201.0230}, 2011.

\bibitem{feifei2020bert}
X. Feifei, Z. Shuting, and Y. Tian,
"Bert-based Siamese network for semantic similarity," 
in \textit{Journal of Physics: Conference Series}, vol. 1684, no. 1, p. 012074, 2020.

\bibitem{cousot1978automatic}
P. Cousot and N. Halbwachs,
"Automatic discovery of linear restraints among variables of a program," 
in \textit{Proc. of the 5th ACM SIGACT-SIGPLAN Symposium on Principles of Programming Languages}, pp. 84--96, 1978.


\bibitem{liu2024enhancing}
R. Liu, G. Li, M. Chen, L.-I. Wu, and J. Ke,
"Enhancing Automated Loop Invariant Generation for Complex Programs with Large Language Models," 
\textit{arXiv preprint arXiv:2412.10483}, 2024.

\bibitem{pirzada2024llm}
M. A. A. Pirzada, G. Reger, A. Bhayat, and L. C. Cordeiro,
"Llm-generated invariants for bounded model checking without loop unrolling," 
in \textit{Proc. of the 39th IEEE/ACM Int. Conf. on Automated Software Engineering}, pp. 1395--1407, 2024.

\bibitem{wu2023lemur}
H. Wu, C. Barrett, and N. Narodytska,
"Lemur: Integrating large language models in automated program verification," 
\textit{arXiv preprint arXiv:2310.04870}, 2023.

\bibitem{brown2020language}
T. Brown, B. Mann, N. Ryder, M. Subbiah, J. D. Kaplan, P. Dhariwal, A. Neelakantan, P. Shyam, G. Sastry, A. Askell, et al.,
"Language models are few-shot learners," 
\textit{Advances in Neural Information Processing Systems}, vol. 33, pp. 1877--1901, 2020.


\bibitem{gao2024customizing}
X. Gao and K. Das,
"Customizing language model responses with contrastive in-context learning," 
in \textit{Proc. of the AAAI Conf. on Artificial Intelligence}, vol. 38, no. 16, pp. 18039--18046, 2024.

\bibitem{hamdan2025much}
S. Hamdan and D. Yuret,
"How much do LLMs learn from negative examples?" 
\textit{arXiv preprint arXiv:2503.14391}, 2025.

\bibitem{sharma2013data}
R. Sharma, S. Gupta, B. Hariharan, A. Aiken, P. Liang, and A. V. Nori,
"A data driven approach for algebraic loop invariants," 
in \textit{Programming Languages and Systems: 22nd ESOP, Proc.}, pp. 574--592, 2013.

\bibitem{gulwani2008program}
S. Gulwani, S. Srivastava, and R. Venkatesan,
"Program analysis as constraint solving," 
in \textit{Proc. of the 29th ACM SIGPLAN Conf. on Programming Language Design and Implementation}, pp. 281--292, 2008.

\bibitem{yoshida2024impact}
L. Yoshida,
"The Impact of Example Selection in Few-Shot Prompting on Automated Essay Scoring Using GPT Models," 
in \textit{Int. Conf. on Artificial Intelligence in Education}, pp. 61--73, 2024.

\bibitem{zhao2024expel}
A. Zhao, D. Huang, Q. Xu, M. Lin, Y.-J. Liu, and G. Huang,
"Expel: LLM agents are experiential learners," 
in \textit{Proc. of the AAAI Conf. on Artificial Intelligence}, vol. 38, no. 17, pp. 19632--19642, 2024.

\bibitem{li2024turning}
Y. Li, P. Yuan, S. Feng, B. Pan, B. Sun, X. Wang, H. Wang, and K. Li,
"Turning dust into gold: Distilling complex reasoning capabilities from LLMs by leveraging negative data," 
in \textit{Proc. of the AAAI Conf. on Artificial Intelligence}, vol. 38, no. 17, pp. 18591--18599, 2024.

\bibitem{zeng2023evaluating}
Z. Zeng, J. Yu, T. Gao, Y. Meng, T. Goyal, and D. Chen,
"Evaluating large language models at evaluating instruction following," 
\textit{arXiv preprint arXiv:2310.07641}, 2023.

\bibitem{ragkhitwetsagul2018comparison}
C. Ragkhitwetsagul, J. Krinke, and D. Clark,
"A comparison of code similarity analysers," 
\textit{Empirical Software Engineering}, vol. 23, pp. 2464--2519, 2018.

\bibitem{ahn2022practical}
S. Ahn, S. Ahn, H. Koo, and Y. Paek,
"Practical binary code similarity detection with BERT-based transferable similarity learning," 
in \textit{Proc. of the 38th Annual Computer Security Applications Conf.}, pp. 361--374, 2022.

\bibitem{huang2024survey}
H.-Y. Huang, Y. Yang, Z. Zhang, S. Lee, and Y. Wu,
"A survey of uncertainty estimation in LLMs: Theory meets practice," 
\textit{arXiv preprint arXiv:2410.15326}, 2024.

\bibitem{chen2024survey}
L. Chen, Q. Guo, H. Jia, Z. Zeng, X. Wang, Y. Xu, J. Wu, Y. Wang, Q. Gao, J. Wang, et al.,
"A survey on evaluating large language models in code generation tasks," 
\textit{arXiv preprint arXiv:2408.16498}, 2024.

\bibitem{wu2024divide}
Z. Wu, H. Bai, A. Zhang, J. Gu, V. G. Vydiswaran, N. Jaitly, and Y. Zhang,
"Divide-or-Conquer? Which Part Should You Distill Your LLM?" 
\textit{arXiv preprint arXiv:2402.15000}, 2024.

\bibitem{reynolds2021prompt}
L. Reynolds and K. McDonell,
"Prompt programming for large language models: Beyond the few-shot paradigm," 
in \textit{Extended abstracts of the 2021 CHI conference on human factors in computing systems}, pp. 1--7, 2021.


==> body/3.Experimetal_Design.tex <==
\section{Empirical Study Setup}

Synthesizing loop invariants is an undecidable inference problem and remains a fundamental challenge in program verification. 
Traditionally, both symbolic reasoning and machine learning-based techniques have been employed to infer loop invariants. 
However, these approaches often face limitations related to scalability, generalizability, and adaptability across diverse program structures. 
Recently, generative large language models (LLMs) have demonstrated strong potential in program synthesis tasks. Prior studies~\cite{chakraborty2023ranking, misu2024towards, kamath2023finding} have shown that LLMs can generate loop invariants directly from program specifications. 
This initial progress in the use of LLM inspired us to dig deep into LLMs' capability in Loop invariant inference. 
% Despite this progress, the quality of the generated invariants remains inconsistent, particularly in low-context or under-specified scenarios such as those commonly found in SyGuS-style benchmarks. 
% For example, Chakraborty~\etal~\cite{chakraborty2023ranking} reported that, on average, an LLM must generate nearly 190 samples per specification to produce a correct invariant. 

% To address these limitations and improve the effectiveness of LLM-based loop invariant synthesis, we explored several enhancement strategies. 
In this study, we explore several well known techniques from LLM research to fully identify and exploit LLM in this problem.
Specifically, we investigated variations of few-shot learning and problem partitioning techniques to identify approaches that yield higher-quality invariants. In the few-shot setting, we analyzed how the number and semantic similarity of provided examples influenced synthesis quality, uncovering key insights into optimal example selection. Furthermore, we evaluated the impact of problem transformation and data augmentation techniques on the robustness and correctness of the generated invariants. Additionally, we investigated a problem partitioning strategy, where complex synthesis tasks are decomposed into smaller sub-problems. We then assessed the ability of LLMs to integrate the solutions of these sub-problems into a complete and coherent final invariant.
\subsection {Benchmark} 
\label{benchmark}
We utilized the Loop Invariant Synthesis benchmark dataset curated by Padhi~\etal~ \cite{padhi2016data}, for this study. This dataset consists of 940 problems formatted in SMT~\cite{alur2013syntax}. The dataset was further analyzed by Chakraborty~\etal~\cite{chakraborty2023ranking}, who identified 429 problems with at least one invariant satisfying all verification conditions. From these 429 problems, we randomly selected 210 problems to evaluate different models. To determine the appropriate sample size for our study, we applied the sample size calculation rule proposed by Uddin~\etal~ \cite{uddin2022empirical}, We determined the sample size using a 98\% confidence level, a 5\% margin of error, and an assumed population proportion of 75\%.
.

\begin{figure*}[!ht]
    \centering
    % \includegraphics[width=0.9\linewidth]{images/prompt_IS.png}
    \includegraphics[width=0.8\linewidth]{figures/prompt1_.drawio.pdf}
    \caption{Prompt Template to generate invariants using a set of instructions using LLM}
    \Description{This figure shows a prompt template designed to generate invariants using instructions with a large language model.}
    \label{fig:prompt_gi}
\end{figure*}

\subsection{Instructions Set: } \label{ssec: GI}
% Successful generation of content using LLM requires designing a perfect set of instructions that reflects the nature of responses \cite{chu2024better}.  
% To identify the instructions, we followed the SyGus \cite{corr18padhi} original work and their invariant generation process to define our instruction set. The instructions we identified are presented in the figure \ref{fig:prompt_gi}. These instructions set with additional rules can define the nature of a loop invariant. 

We developed a set of instructions to guide the LLM models about the problem domain-specific knowledge. To create these instructions, we studied the invariant generation process from different state-of-the-art research \cite{padhi2016data, achiam2023gpt, chakraborty2023ranking, wu2023lemur, misu2024towards}, translated the process into structured guidelines, and organized them into a set of instructions for LLM. 

Figure \ref{fig:prompt_gi} illustrates a prompt template containing a set of Instructions. These instructions are composed of three main parts: 1) In the first part (first four lines) of the template, we introduced the problem and defined LLM's role here. 2) The second part is presented as a numbered list of instructions. It guides about the key concerns to be considered while generating the invariants, and the logical consequences to maintain. 3) The third part defines additional rules that constrain LLMs to generate invariants using only the specified variables. We call these instructions together as General Instructions(GIs). 

\subsection{Similarity Measurement Algorithms}
\label{ssec: algo}


\begin{table*}[!t]
    \caption{Comparison of Similarity Measure}
    \centering
    \footnotesize{
    \begin{tabular}{c|c|c}
        \textbf{Query Problem} & \textbf{Example Picked by $\mathcal{S}_{semantic}$} & \textbf{Example Picked by $\mathcal{S}_{syntactic}$} \bigstrut \\
        \hlineB{2}

         \includegraphics[width=0.3\linewidth]{figures/table_codes_q.pdf}
         &          \includegraphics[width=0.3\linewidth]{figures/table_codes_sem.pdf} 
          &        \includegraphics[width=0.3\linewidth]{figures/table_codes_syn.pdf} \bigstrut \\
          \hlineB{2}
    \end{tabular}
    }
    \label{tab: similarity}
\end{table*}

% Given the challenges of synthesizing correct invariants from problem specifications, we explored few-shot prompting as a means to enhance LLM performance in invariant generation. In this approach, prompts were constructed using example problems paired with their corresponding loop invariants. To ensure the relevance of these examples, we selected problems that closely matched the target (query) problem. For problems with program specifications, similarity can be measured using different algorithms. Ragkhitwetsagul ~\etal \cite{ragkhitwetsagul2018comparison} showed that two popular measurement approaches: i) text-based, and ii) tree-based, can be effective in source code similarity computation. From a text-based approach, we select the Web STS BERT\footnote{https://pypi.org/project/semantic-text-similarity/} model, which is one of the most performing BERT-based models for semantic similarity measurement\cite{ahn2022practical}. On the other hand, from the tree-based models we selected APTED\footnote{https://pypi.org/project/apted/}, an algorithm that measures syntactic similarity based on Abstract Syntax Trees (AST). We evaluated the performance of these models by assessing the success rate of LLMs using examples identified by each similarity measurement method.


% Given the challenges of synthesizing correct invariants from problem specifications, 

To assess LLMs' ability to synthesize loop invariants, we use in-context learning with few-shot prompts composed of example problems and their invariants. 
To ensure relevance, we select examples similar to the target problem using established similarity metrics. 
For text-based similarity ($\mathcal{S}_{semantic}$), we apply the Web STS BERT model\footnote{\url{https://pypi.org/project/semantic-text-similarity/}}~\cite{ahn2022practical}; for tree-based similarity ($\mathcal{S}_{syntactic}$), we use APTED\footnote{\url{https://pypi.org/project/apted/}} over ASTs~\cite{ragkhitwetsagul2018comparison}. 
We evaluate these methods by measuring the success rate of LLM-generated invariants using examples selected by each of these similarity metrics. We discussed the result in Table ~\ref{tab:fewshot_performance}. 
% \saikat{forward reference to the table where you show this result.}.


% To fully test LLMs' capabilities in synthesizing invariant, we explored in context learning by few-shot prompting. 
% In this approach, prompts were constructed using example problems paired with their corresponding loop invariants. 
% To ensure the relevance of these examples, we selected problems that closely matched the target (query) problem. 
% For problems described through program specifications, similarity between the query and candidate examples was measured using established similarity computation techniques. 
% Ragkhitwetsagul~\etal~\cite{ragkhitwetsagul2018comparison} demonstrated that two commonly used approaches: (i) text-based and (ii) tree-based, are effective in measuring source code similarity. 
% For the text-based similarity ($\mathcal{S}_{semantic}$), we used the Web STS BERT model\footnote{\url{https://pypi.org/project/semantic-text-similarity/}}, a high-performing BERT-based model for semantic similarity measurement~\cite{ahn2022practical}. 
% For the tree-based similarity measurement ($\mathcal{S}_{syntactic}$) we leveraged APTED\footnote{\url{https://pypi.org/project/apted/}}, an algorithm that computes syntactic similarity based on Abstract Syntax Trees (ASTs). 
% We evaluated the effectiveness of these similarity models by measuring the success rate of LLM-generated invariants when using examples selected by each method.



\paragraph{$\mathcal{S}_{semantic}$ : }

Given a problem $\mathcal{P}$, we generate the vector embedding of that $Emb_{\mathcal{P}}$. Then, we compute the cosine similarity of all other problems ($\mathcal{Q}_i$) embedding $Emb_{\mathcal{Q}_i}$, and select the top $k$ problems (and their corresponding ground truth invariants) as few shot examples. 

% In this work, we refer to the Web STS BERT-based similarity measurement technique as $\mathcal{S}_{semantic}$. This model computes the semantic similarity between two input problem descriptions and returns a numerical score ranging from 0 to 5. For a given query problem, we compute similarity scores against all other problems in the dataset and rank them accordingly. The top-ranked problems, i.e., those most similar to the query, are selected as \emph{example problems} in the context of few-shot prompting. In \cref{tab: similarity}, the column titled "Example picked by $\mathcal{S}_{semantic}$" presents the example problem that received the highest similarity score relative to the query problem, as determined by the $\mathcal{S}_{semantic}$ method.




\paragraph{$\mathcal{S}_{syntactic}$ : }
Computing $\mathcal{S}_{syntactic}$ is more involved than $\mathcal{S}_{semantic}$. Given a problem $\mathcal{P}$ and a candidate $\mathcal{Q}_i$, we parse their precondition ({\tt PreF}), postcondition ({\tt PostF}), and transfer function ({\tt TransF}) into ASTs, and compute APTED similarity between each corresponding pair (\eg, $PreF_{\mathcal{P}}$ vs.\ $PreF_{\mathcal{Q}_i}$). The overall similarity is the mathematical sum 
% \saikat{Sum? Mean?} 
of the three function-level similarities. Similar to $\mathcal{S}_{semantic}$, we select the top-$k$ most similar problems for few-shot prompting.

\Cref{tab: similarity} illustrates a query problem $\mathcal{P}$ and its top matches under both similarity metrics. $\mathcal{S}_{semantic}$ favors surface-level matches, often selecting examples with identical method names but differing logic. In contrast, $\mathcal{S}_{syntactic}$ captures deeper structural similarity, identifying semantically similar programs even when identifiers differ.

% This method of similarity calculation is slightly more involved than $\mathcal{S}_{semantic}$. To compute the similarity between a given problem $\mathcal{P}$, and any other problem in the dataset $\mathcal{Q}_i$, we parse the problems and extract the ASTs corresponding to precondition ({\tt PreF}), postcondition ({\tt PostF}), and Transfer Function ({\tt TransF}) from both of the problems. We then compute the AST similarity (using APTED) between each pair of functions (\eg $PreF_{\mathcal{P}}$ and $PreF_{\mathcal{Q}_i}$). We then compute the similarity between the problems $\mathcal{P}$ and $\mathcal{Q}_i$ by aggregating \saikat{what do you mean by aggregate? Sum? Mean?} the similarities between {\tt PreF}, {\tt TransF}, and {\tt PostF}. Similar to $\mathcal{S}_{semantic}$, we select top k problems for showing as in-context examples in the prompt. 

% We refer to the AST-based similarity measurement technique as $\mathcal{S}_{syntactic}$. This approach takes two problems as input and analyzes the syntactic structure of their corresponding functions (e.g., \texttt{PreF}, \texttt{TransF}) by converting them into Abstract Syntax Trees (ASTs). For each pair of corresponding functions, the method constructs their AST representations and compares them using a node-level matching strategy. Each matched node contributes one point to the similarity score. The scores from all four functional components are then aggregated to compute a total syntactic similarity score between the two problems.

% As with $\mathcal{S}_{semantic}$, each query problem is compared against all others in the dataset, and the problems are ranked based on their total similarity scores. The highest-ranked problems are considered the most syntactically similar and are selected as example problems. In \cref{tab: similarity}, the column labeled "Example picked by $\mathcal{S}_{syntactic}$" shows the example problem that achieved the highest similarity score with the query problem according to this method.

% \cref{tab: similarity} shows an example of a problem being solved (as Query Problem $\mathcal{P}$), and top problem selected by $\mathcal{S}_{semantic}$, and $\mathcal{S}_{syntactic}$.
% % A closer examination of the examples selected by each algorithm in \cref{tab: similarity} reveals distinct characteristics in their similarity assessments. 
% Upon closer observation to the problems selected by each of these similarity metrics, we notice that the $\mathcal{S}_{semantic}$ method tends to emphasize string-level matching; it often selects examples where method names (\eg \texttt{PreF}, \texttt{TransF}) are identical, even when the underlying operations differ significantly. 
% In contrast, $\mathcal{S}_{syntactic}$ places greater emphasis on the structural similarity of operations, often identifying examples with similar program logic despite differences in method naming.

\begin{table*}[!t]
    \centering
    \caption{Different types of Examples}
    \footnotesize{
     % \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{m{0.1\linewidth}|m{0.7\linewidth}}
        \textbf{Type} & \textbf{Example}  \bigstrut \\ 
        \hlineB{2} \\
         $\mathcal{EX}_{P}$ & \includegraphics[width=\linewidth]{figures/examples_p.drawio.pdf}
         \bigstrut \\
         $\mathcal{EX}_{N}$ & \includegraphics[width=\linewidth]{figures/examples_n.drawio.pdf} \bigstrut \\
         $\mathcal{EX}_{Mix}$ & \includegraphics[width=\linewidth]{figures/examples_mix.drawio.pdf} \bigstrut \\
         \hlineB{2}
    \end{tabular}    
    }
    \label{tab:examples}
\end{table*}

\begin{figure*} [!t]
    \centering
    % \includegraphics[width=0.9\linewidth]{images/few_shot_template.jpg}
    \includegraphics[width=0.75\linewidth]{figures/prompt_few_shot.drawio.pdf}
    % \caption{Prompt Template to generate invariants using Few shot examples} \saikat{Remove the word SyGus from prompt}}
    \label{fig:few-shot-template}
\end{figure*}

\subsection{Types of Examples in Few-shot} \label{ssec: examples}
The primary philosophy behind in-context learning~\cite{brown2020language} is to show LLM some illustration of how a task is performed. 
In a way, such prompting strategy is to guide model on {\em what to do}. 
Few recent works~\cite{hamdan2025much, gao2024customizing} also investigated LLMs' responses when provided with negative example, guiding the LLMs on {\em what not to do}. 
Inspired by these works, we investigated addition pf three types of few shot examples in the prompt. 

\paragraph{ $\mathcal{EX}_{P}$ (Positive example) : } 
A positive example consists of a problem paired with an invariant that satisfies the specification. 

\paragraph{ $\mathcal{EX}_{N}$ (Negative example) : }
A negative example is an invariant synthesis problem, a candidate invariant that fails to satisfy the specification, and the reason for this failure. 

\paragraph{ $\mathcal{EX}_{Mix}$ (Mixed example) : } The Mixed example is composed of both satisfying and unsatisfying invariants of a problem.

\Cref{tab:examples} shows examples of  of $\mathcal{EX}_{P}$, $\mathcal{EX}_{N}$, and $\mathcal{EX}_{Mix}$ and how we present them in the prompt.


% An example of $\mathcal{EX}_{Mix}$ is shown in  ~\Cref{tab:examples}. 
% These types of examples are useful for training the LLM to distinguish between valid and invalid invariants within the same problem context. 
% These examples are intended to help the LLM learn to avoid patterns that lead to invalid invariants for a given problem.


% In \Cref{ssec: algo}, we devised the example problems selection process using similarity algorithms. The benchmark dataset contains problem specifications, synthesized invariants, and corresponding verification results for each of the invariants. We compose a complete example ($\mathcal{EX}$) with a problem and its invariant(s). Based on verification status of the invariant, an $\mathcal{EX}$ can be of one of the three possible types types - 1) $\mathcal{EX}_{P}$ 2) $\mathcal{EX}_{N}$ and 3)  $\mathcal{EX}_{Mix}$


% \subsubsection{ $\mathcal{EX}_{P}$ (Positive example):} 
% A positive example consists of an SMT problem paired with an invariant that correctly satisfies the specification. \Cref{tab:examples} illustrates a typical $\mathcal{EX}_{P}$, showing one problem along with its valid invariant. These examples are designed to help the LLM identify the patterns associated with correct invariants for specific problems.


\subsection{Experimental Workflow}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/llm4liProcess.drawio.pdf}
    \caption{General workflow of the experiment}
    \label{fig:model}
\end{figure}

~\Cref{fig:model} illustrates the generic workflow of our experiments. 
The process starts with a query invariant synthesis problem $\mathcal{P}$ represented in SMT format. 
Based on the query, the system constructs a prompt using one of several prompt builders (shown as \textbf{RQ1.*} boxes in ~\cref{fig:model}) and sends it to an LLM, which generates candidate invariants. 
The invariant parser extracts these invariants from the LLM’s output and forwards them to the verifier (Z3) to check against the problem’s verification conditions. 
If the verifier can prove the correctness of an invariant, the system accepts it. 
Otherwise, it creates a repair prompt using the verifier’s feedback and asks the LLM to revise the invariant. 
The system then re-parses and re-verifies the revised output. 
This cycle continues until the system finds a valid invariant or terminates after repeated failures.



% ~\Cref{fig:model} illustrates the workflow of the proposed experimental framework. The process begins with a query problem for which an invariant is to be synthesized. Based on this query, the system constructs a prompt using one of several prompt builders, represented by the \textbf{RQ1.*} boxes in ~\cref{fig:model}. This prompt is then provided to an LLM, which generates candidate invariants in response. An invariant parser extracts the generated invariants from the LLM's output. Each extracted invariant is passed to a verifier (Z3), which checks whether it satisfies the verification conditions of the problem. If the invariant passes verification, it is marked as successful. If it fails, the system constructs a repair prompt that includes the verifier’s feedback. The LLM then attempts to revise the invariant based on this feedback. The revised invariant is again processed by the parser and submitted to the verifier. This cycle continues until a successful invariant is produced or the process is terminated due to repeated failure.

% \todo{

% thee part 
% general problem structure
% how to approach the problem
% rules to follow
% }

% \begin{itemize}

%     \item Make a note of the conditions in the problem.
%     \item Analyze the problem and make a note of the conditions.
%     \item Output invariants that are true
%     \begin{itemize}
%         \item before the loop execution (pre-function)
%         \item in every iteration of the loop and (trans function)
%         \item	after the loop termination (post-function).
%     \end{itemize}
% \end{itemize}
% In addition to the instruction set, we add some rules to be followed for the generated invariants. Which are - 
% \begin{itemize}
%     \item Do not use variables or functions which are not declared in the problem.
%     \item Do not make any assumptions about functions whose definitions are not given.
%     \item All undefined variables contain garbage values. Do not use variables that have garbage values.
%     \item Variables that are not explicitly initialized could have garbage values. Do not make any assumptions about such values.
%     \item Do not use non-deterministic function calls.
% \end{itemize}


% \begin{table*}[h]
%  \caption{Comparison of Similarity Measure}
%     \centering
% %     \begin{tabular}{  | p{0.31\linewidth} | p{0.31\linewidth} | p {0.31\linewidth} |} \hline 
% %          Original Problem &  Similar Problem Capture by AST distance& Similar Problem Captured by BERT\\ \hline 
% %      \begin{lstlisting}
% % (set-logic LIA)

% % (synth-inv inv_fun ((i Int) (t Int) (x Int) (y Int)))

% % (define-fun pre_fun ((i Int) (j Int) (n Int) (k Int)) Bool
% %     (and (or (= n 1) (= n 2)) (= i 0) (= j 0)))
% % (define-fun trans_fun ((i Int) (j Int) (n Int) (k Int) (i! Int) (j! Int) (n! Int) (k! Int)) Bool
% %     (or (and (> i k) (= i! i) (= j! j) (= n! n) (= k! k)) (and (<= i k) (= i! (+ i 1)) (= j! (+ j n)) (= n! n) (= k! k))))
% % (define-fun post_fun ((i Int) (j Int) (n Int) (k Int)) Bool
% %     (=> (> i k) (or (not (= n 1)) (= i j))))

% % (inv-constraint inv_fun pre_fun trans_fun post_fun)

% % (check-synth)

% % \end{lstlisting}
       
% %        & 
% % \begin{lstlisting}
% % (set-logic LIA)

% % (synth-inv inv_fun ((i Int) (t Int) (x Int) (y Int)))

% % (define-fun pre_fun ((i Int) (t Int) (x Int) (y Int)) Bool
% %     (and (not (= x y)) (= i 0) (= t y)))
% % (define-fun trans_fun ((i Int) (t Int) (x Int) (y Int) (i! Int) (t! Int) (x! Int) (y! Int)) Bool
% %     (or (and (> x 0) (= i! i) (= t! t) (= x! x) (= y! (+ x y))) (and (<= x 0) (= i! i) (= t! t) (= x! x) (= y! y))))
% % (define-fun post_fun ((i Int) (t Int) (x Int) (y Int)) Bool
% %     (>= y t))
    

% % (inv-constraint inv_fun pre_fun trans_fun post_fun)

% % (check-synth)
% % \end{lstlisting}
       
% %        & 
% % \begin{lstlisting}
% % (set-logic LIA)

% % (synth-inv InvF ((n Int) (i Int) (k Int) (j Int)))

% % (define-fun PreF ((n Int) (i Int) (k Int) (j Int)) Bool
% %     (and (= i 0) (= k 0) (= j 0)))
% % (define-fun TransF ((n Int) (i Int) (k Int) (j Int) (n! Int) (i! Int) (k! Int) (j! Int)) Bool
% %     (or (and (< i n) (= i! (+ i 1)) (= k! (+ k 1)) (= n! n) (= j! j)) (and (>= i n) (< j n) (= j! (+ j 1)) (= k! (- k 1)) (= n! n) (= i! i))))
% % (define-fun PostF ((n Int) (i Int) (k Int) (j Int)) Bool
% %     (or (not (and (>= i n) (< j n))) (> k 0)))

% % (inv-constraint InvF PreF TransF PostF)

% % (check-synth)
% %        \end{lstlisting}
       
% %        \\ \hline 
% %     \end{tabular}

%         % \begin{figure*}[!t]
%             \centering
%             \includegraphics[width=\linewidth]{figures/table_codes.drawio.pdf}
%             % \caption{Caption}
%             % \label{fig:enter-label}
%         % \end{figure*}
   
%     \label{tab: similarity}
% \end{table*}

% \subsection{Similarity Measurement Algorithms}
% \label{ssec: algo}

% % Given the challenges of synthesizing correct invariants from problem specifications, we explored few-shot prompting as a means to enhance LLM performance in invariant generation. In this approach, prompts were constructed using example problems paired with their corresponding loop invariants. To ensure the relevance of these examples, we selected problems that closely matched the target (query) problem. For problems with program specifications, similarity can be measured using different algorithms. Ragkhitwetsagul ~\etal \cite{ragkhitwetsagul2018comparison} showed that two popular measurement approaches: i) text-based, and ii) tree-based, can be effective in source code similarity computation. From a text-based approach, we select the Web STS BERT\footnote{https://pypi.org/project/semantic-text-similarity/} model, which is one of the most performing BERT-based models for semantic similarity measurement\cite{ahn2022practical}. On the other hand, from the tree-based models we selected APTED\footnote{https://pypi.org/project/apted/}, an algorithm that measures syntactic similarity based on Abstract Syntax Trees (AST). We evaluated the performance of these models by assessing the success rate of LLMs using examples identified by each similarity measurement method.


% Given the challenges of synthesizing correct invariants from problem specifications, we explored few-shot prompting as a means to enhance the performance of large language models (LLMs) in invariant generation. In this approach, prompts were constructed using example problems paired with their corresponding loop invariants. To ensure the relevance of these examples, we selected problems that closely matched the target (query) problem. For problems described through program specifications, similarity between the query and candidate examples was measured using established similarity computation techniques. Ragkhitwetsagul~\etal~\cite{ragkhitwetsagul2018comparison} demonstrated that two commonly used approaches: (i) text-based and (ii) tree-based, are effective in measuring source code similarity. For the text-based method, we adopted the Web STS BERT model\footnote{\url{https://pypi.org/project/semantic-text-similarity/}}, a high-performing BERT-based model for semantic similarity measurement~\cite{ahn2022practical}. For the tree-based method, we selected APTED\footnote{\url{https://pypi.org/project/apted/}}, an algorithm that computes syntactic similarity based on Abstract Syntax Trees (ASTs). We evaluated the effectiveness of these similarity models by measuring the success rate of LLM-generated invariants when using examples selected by each method.



% \subsubsection{Semantic Similarity}

% In this work, we refer to the Web STS BERT-based similarity measurement technique as $\mathcal{S}_{semantic}$. This model computes the semantic similarity between two input problem descriptions and returns a numerical score ranging from 0 to 5. For a given query problem, we compute similarity scores against all other problems in the dataset and rank them accordingly. The top-ranked problems, i.e., those most similar to the query, are selected as \emph{example problems} in the context of few-shot prompting. In \cref{tab: similarity}, the column titled "Example picked by $\mathcal{S}_{semantic}$" presents the example problem that received the highest similarity score relative to the query problem, as determined by the $\mathcal{S}_{semantic}$ method.




% \subsubsection{Syntactic Similarity}
% We refer to the AST-based similarity measurement technique as $\mathcal{S}_{syntactic}$. This approach takes two problems as input and analyzes the syntactic structure of their corresponding functions (e.g., \texttt{PreF}, \texttt{TransF}) by converting them into Abstract Syntax Trees (ASTs). For each pair of corresponding functions, the method constructs their AST representations and compares them using a node-level matching strategy. Each matched node contributes one point to the similarity score. The scores from all four functional components are then aggregated to compute a total syntactic similarity score between the two problems.

% As with $\mathcal{S}_{semantic}$, each query problem is compared against all others in the dataset, and the problems are ranked based on their total similarity scores. The highest-ranked problems are considered the most syntactically similar and are selected as example problems. In \cref{tab: similarity}, the column labeled "Example picked by $\mathcal{S}_{syntactic}$" shows the example problem that achieved the highest similarity score with the query problem according to this method.

% A closer examination of the examples selected by each algorithm in \cref{tab: similarity} reveals distinct characteristics in their similarity assessments. The $\mathcal{S}_{semantic}$ method tends to emphasize string-level matching; it often selects examples where method names (\eg \texttt{PreF}, \texttt{TransF}) are identical, even when the underlying operations differ significantly. In contrast, $\mathcal{S}_{syntactic}$ places greater emphasis on the structural similarity of operations, often identifying examples with similar program logic despite differences in method naming.


% We devised two similarity finding algorithms. Referring back to the problem and similar examples discussed in the Table \ref{tab: similarity}, the example picked by AST-based syntactic algorithm has a ground truth invariant {\texttt{(or (and (= x 1) (= y 0)) (= x 0))}} and the example picked by BERT-based semantic algorithm has the ground truth invariant {\texttt{(and (or (= x 100) (>= y 0)) (or (= x 99) (not (= 0 y))) (or (>= y x) (= (+ x y) 99)) ...)}}. 
% Designing a prompt to generate invariants for the query problem mentioned in the table, composing few-shot with each of the examples, GPT-4o responded with invariants {\texttt{(or (= x 0) (< y 1024))}}, and {\texttt{(and (or (= x 1) (= y 0)) (or (not (= x 0)) (< y 1024)) ...)}} respectively. 
% The first one was a successful invariant, and the second one failed to satisfy the verifier. That motivated us to explore the case more deeply. 
% In this section, we discussed the detailed analysis of the impact of similarity measures in the few-shot prompting. \todo{move the details in section 3 }


% \begin{table*}[!t]
%     \centering
%     \caption{Different types of Examples}
%     \footnotesize{
%      % \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{m{0.1\linewidth}|m{0.7\linewidth}}
%         \textbf{Type} & \textbf{Example}  \bigstrut \\ 
%         \hlineB{2} \\
%          $\mathcal{EX}_{P}$ & \includegraphics[width=\linewidth]{figures/examples_p.drawio.pdf}
%          \bigstrut \\
%          $\mathcal{EX}_{N}$ & \includegraphics[width=\linewidth]{figures/examples_n.drawio.pdf} \bigstrut \\
%          $\mathcal{EX}_{Mix}$ & \includegraphics[width=\linewidth]{figures/examples_mix.drawio.pdf} \bigstrut \\
%          \hlineB{2}
%     \end{tabular}    
%     }
%     \label{tab:examples}
% \end{table*}

% \subsection{Types of Examples in Few-shot} \label{ssec: examples}

% In \Cref{ssec: algo}, we devised the example problems selection process using similarity algorithms. The benchmark dataset contains problem specifications, synthesized invariants, and corresponding verification results for each of the invariants. We compose a complete example ($\mathcal{EX}$) with a problem and its invariant(s). Based on verification status of the invariant, an $\mathcal{EX}$ can be of one of the three possible types types - 1) $\mathcal{EX}_{P}$ 2) $\mathcal{EX}_{N}$ and 3)  $\mathcal{EX}_{Mix}$


% \subsubsection{ $\mathcal{EX}_{P}$ (Positive example):} 
% A positive example consists of an SMT problem paired with an invariant that correctly satisfies the specification. \Cref{tab:examples} illustrates a typical $\mathcal{EX}_{P}$, showing one problem along with its valid invariant. These examples are designed to help the LLM identify the patterns associated with correct invariants for specific problems.

% \subsubsection{ $\mathcal{EX}_{N}$ (Negative example):}
 
%  A negative example consists of an SMT problem, an invariant that fails to satisfy the specification, and the reason for this failure. \Cref{tab:examples} presents an instance of $\mathcal{EX}_{N}$. These examples are intended to help the LLM learn to avoid patterns that lead to invalid invariants for a given problem.


% \subsubsection{ $\mathcal{EX}_{Mix}$ (Mixed example):} The Mixed example is composed of both satisfying and unsatisfying invariants of a problem. An example of $\mathcal{EX}_{Mix}$ is shown in  ~\Cref{tab:examples}. These types of examples are useful for training the LLM to distinguish between valid and invalid invariants within the same problem context. 

% \subsection{Prompt Design} \label{ssec:pd}
% To prompt with LLM, we started designing the system from two perspectives. Firstly, we tried to prompt LLM with a set of instructions that could guide LLM to generate invariants following the problem context. Secondly, for the few-shot prompting, design a template that can utilize the examples to produce loop invariants. In the case of few-shot examples, we conducted several studies to find the best combination. The combinations we tried - 
% \begin{itemize}
%     \item Few-shot with correct invariants only, correct invariants denote the invariants that complete the verification with the corresponding problem.  
%     \item Few-shot with incorrect invariants only, incorrect invariants denote the invariants that couldn't satisfy all the verification conditions. LLMs were asked to analyze the incorrect invariant and restrict the production of invariants that can similarly violate the verification conditions.    
%     \item Few-shot with the mix of correct and incorrect invariants.  
% \end{itemize}

% Figure \ref{fig:prompt_gi} represents the prompt designed to find the invariants with the general instruction set. In this prompt, we include the original problem and one example output invariant format to guide the LLM. Figure \ref{fig:few-shot-template} represents the general template of the few-shot prompt. According to the model of prompting the problem, the invariant function's signature, similar problems, and invariants were placed into the template. In this study, most of the experiments were conducted using the template represented in Figure \ref{fig:few-shot-template}. In the case of negative invariant examples, we included the description of failure to satisfy the conditions. 
% \todo{seems outdated}

% \begin{figure*} [!t]
%     \centering
%     % \includegraphics[width=0.9\linewidth]{images/few_shot_template.jpg}
%     \includegraphics[width=0.75\linewidth]{figures/prompt_few_shot.drawio.pdf}
%     \caption{Prompt Template to generate invariants using Few shot examples}
%     \label{fig:few-shot-template}
% \end{figure*}

% % \subsection{Research Questions}

% % \RQ{1} {Can a prompt with the Generalized Instructions (GI) set help LLM to generate an inductive loop invariant for a low-level computer program?}

% % Existing invariant synthesize studies \cite{chakraborty2023ranking} showed LLM could produce inductive loop invariants based on presented instructions. However, adequate fine-tuning, a large sample generation, and extensive testing are required. We have created an instruction set and found that GPT-4o can generate loop invariants following the instructions.  

% % \RQ{2} {Can a few-shot be applied for inductive loop invariant generation?}

% % Examples of similar problems and their corresponding invariants can help LLM generate better invariants. Finding similar problems is also challenging. For a sygus like programming, it is difficult to define the similarity of the problems. We performed AST tree-based similarity on top of participating variable counts. Enclosing more than one similar problem and corresponding invariant improves the performance of LLM in the quality of invariants. 

% % Attaching the examples in the prompt can guide LLM to produce more accurate results. In the context of this study, only providing some invariant examples is not sufficient, rather, we need to find appropriate examples to follow. To decide on appropriate examples, we examine test cases- 1) Find the semantically similar sygus problems with positive invariants and prompt LLM with those invariant examples. 2) Prompt with semantically similar positive and negative invariants. 
% % 3) Determine similar problems with distance tree-based structures and prompt them by attaching the positive invariants
% % 4) In the top of the tree distance, we have applied the constraint on the number of parameters. Only the problems with the same number of variables as the seed problem were considered for similar problem candidates. 

% % Our experiments indicate that among the four variations of the few shots, the fourth one performs the best.  On the other hand, providing the negative examples is the less performing variation.  

% % \RQ{3} {Is combining the GI and few-shot in prompt perform better?} 

% % We have generated the prompts with general instructions and few-shot examples to examine if the performance of the LLM improves. Unfortunately, our experiments could not find better results with the prompts containing both general instructions and few-shot examples.

% % \RQ{4} {Can LLM repair the incorrect invariants by analyzing the information of failure?} 

% % Once the produced invariant is tested with the Z3 library, it returns either pass or fail status. For the failed cases, we have explored the log and extracted the model to identify the condition that fails with corresponding model values. We re-prompted the LLM with the negative-invariant, unsatisfied condition and corresponding values for which it failed. Experiments show that it can not help LLM a lot. LLM shows success in repair in one out of three cases. 

% % \RQ{5} {Can break the query problem into sub-problems help LLM to generate better invariants?}

% % The sygus problem contains four methods called pre-function, post-function, transition-function, and invariant-function. And for the invariant, it needs to satisfy the following three conditions -  1) pre-function implies invariant-function, 2) (transition-function and invariant-function) implies transition-function, and 3) invariant-function implies post-function. We break the invariant generation problem into three parts based on the satisfy-ability conditions.  First, prompt LLM to produce several extensive invariants that satisfy condition 1, then similarly for condition two and condition 3. After getting those partial invariants, I asked LLM to merge them into a single minimal invariant that covers all the given conditions. This process also fails to produce satisfactory invariants either.  

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/llm4liProcess.drawio.pdf}
%     \caption{General workflow of the experiment}
%     \label{fig:model}
% \end{figure}

% \subsection{Workflow of the experimental study}


% % The workflow of the experimental system model is presented in Figure \ref{fig: model}. The system takes the seed problem as input, and using the prompt generator, it prepares the required prompt. In the Prompt Generator (PG), a similar problem finder communicates with the invariant database to find the most likely problems to use as examples in the few-shot prompt. The similar problem finder uses either a base semantic similarity model or an AST tree-based distance model to rank the most similar problems. After finding the top n (n, any user-defined parameter) similar problems, the PG uses the prompting templates to generate the prompts. With the generated prompt, the system triggers LLM to generate the responses. In this step, we set the necessary LLM parameters to get the best possible outputs. After getting the responses (top k invariants) from the language model, it requires some processing to extract the invariant from unstructured response text. The Invariant Extractor reads the response text and extracts the invariants for further verification.  

% Figure ~\ ref{fig:model} illustrates the workflow of the proposed experimental framework. The process begins with a query problem for which an invariant is to be synthesized. Based on this query, the system constructs a prompt using one of several prompt builders, represented by the \textbf{RQ1.*} boxes in ~\cref{fig:model}. This prompt is then provided to an LLM, which generates candidate invariants in response. An invariant parser extracts the generated invariants from the LLM's output. Each extracted invariant is passed to a verifier (Z3), which checks whether it satisfies the verification conditions of the problem. If the invariant passes verification, it is marked as successful. If it fails, the system constructs a repair prompt that includes the verifier’s feedback. The LLM then attempts to revise the invariant based on this feedback. The revised invariant is again processed by the parser and submitted to the verifier. This cycle continues until a successful invariant is produced or the process is terminated due to repeated failure.

==> body/4.Results.tex <==
\section{Results}
% \saikat{Rewrite things in active voice}
% The experiment on the sygus dataset\saikat{the dataset is not called SyGus dataset} was conducted in several open-source and proprietary LLMs.

 % We conduct the experiment on the Loop Invariant Synthesis benchmark dataset, organized by Padhi et al. \cite{padhi2016data}. The dataset contains 940 problems in SyGus \cite{alur2013syntax} format. In our experiment, we asked differnt LLMs to produce a set of satisfying invariants, \textbf{\textit{I}} = \{ $I_1$, $I_2$, $I_3$, ...., $I_K$ \} for the given problem \textbf{\textit{P}}, where $K$ is a user-defined number to control the number of invariants produced by LLM. The generated invariants were tested using the \textit{lig-verify} library prepared by \cite{corr18padhi}.   
We answer the following major research questions (RQs):
\begin{enumerate}[label=\textbf{RQ\arabic{*}.}]
    \item How good are LLMs at generating loop invariants from program specifications?
    \item Can LLMs repair their incorrect loop invariants?
\end{enumerate}
We used the SMT-formatted benchmark dataset that we introduced in Section \ref{benchmark}. We studied three LLMs: one closed-source (GPT-4o \cite{achiam2023gpt}), and two open-source (Mistral-large \cite{mistral_large} and Llama 3.1 (8B) \cite{meta2024llama3}).
 % In this section, we present a comprehensive analysis of the research questions, including their motivations, the experiments conducted, the outcomes of these experiments, and further discussions. To prepare the results, we evaluated the benchmark dataset (described in \ref{benchmark}), using three large language models (LLMs): one closed-source model, GPT-4o \cite{achiam2023gpt}, and two open-source models, Mistral-large \cite{mistral_large} and Llama 3.1 (8B) \cite{meta2024llama3}.


\subsection{ [RQ1] How good are LLMs at generating loop invariants from program specification?}

% To examine the LLM's ability to generate loop invariants for low-level program specifications, we designed this experiment. We examined three popular LLM models, GPT-4o, Mistral-large and Llama3.1 (8B) in this setup. \todo{why these three- ref/benchmark presentation-mostafij}. 

While LLMs have demonstrated proficiency in generating code from program specifications \cite {chen2024survey},  
their effectiveness in generating loop invariants is relatively underexplored. 
% their effectiveness in generating loop invariants from low-level program specifications is not studied. 
Our study aims at exploring such capability with comprehensivity. 
Concretely, for each LLM, we explored various prompting strategies to produce the invariants. We examine the invariants and the ability of the LLM to follow the prompts properly. We answer three sub-RQs:
% Beyond merely testing their capability to produce loop invariants, we also examine their ability to follow instructions and generate invariants that satisfy validation conditions. 
% From these perspectives, we further decompose \textbf{RQ1} into three sub-questions

\begin{itemize}
    \item \textbf{[RQ1.1]} Can LLMs generate loop invariants following the provided domain knowledge? 
    \item \textbf{[RQ1.2]} Can LLMs generate loop invariants by learning from similar examples?   
    \item \textbf{[RQ1.3]} Is the integration of domain knowledge and similar examples more useful for LLM to produce loop invariants?
\end{itemize}



\subsubsection{[RQ1.1]} Can LLMs generate loop invariants following the provided domain knowledge?

\begin{table}[!t]
\caption{Study on LLMs' Invariant Generation Capability}
\label{tab: GIcomparision}
\footnotesize
\centering
% \begin{tabular}{p{.10\linewidth}|p{.18\linewidth}|p{.15\linewidth}|p{.17\linewidth}|p{.20\linewidth}|}
% % \hline
% \textbf{LLM} & \textbf{Generated invariant} & \textbf{Followed output template} & \textbf{Automated extracted invariant} & \textbf{Syntactically correct} \\
% \hline
% llama 3.1 8b & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} \\
% \hline
% Mistral-large & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{25} & \multicolumn{1}{c|}{25} & \multicolumn{1}{c|}{22} \\
% \hline
% GPT-4o & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c|}{30} \\
% \hline

\begin{tabular}{l|l|l}
% \hline
\textbf{LLM} & \textbf{\# Followed template}  & \textbf{\# Syntactically correct} \\
\hlineB{2}
\textbf{Llama 3.1 8b} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c}{0} ~\bigstrut\\
\hline
\textbf{Mistral-large} & \multicolumn{1}{c|}{25} & \multicolumn{1}{c}{22} ~\bigstrut \\
\hline
\textbf{GPT-4o} & \multicolumn{1}{c|}{30} & \multicolumn{1}{c}{30} ~\bigstrut \\
\hlineB{2}
\end{tabular}
\end{table}




\motivation
% LLMs represent a valuable source of multidimensional knowledge. 
% In this context, we are referring domain knowledge as the essential background regarding the problem, the characteristics of potential solutions, and the verification processes needed to validate those solutions.

% Large Language Models are useful for many different tasks when instructed properly~\cite{chang2024survey}.
% To effectively guide these models in generating content for specific tasks, we can supply them with domain knowledge~\cite{zeng2023evaluating}. 

Large Language Models (LLMs) have demonstrated strong capabilities across a variety of tasks when given appropriate instructions~\cite{chang2024survey}. However, their effectiveness can be limited in domains that require deep reasoning or specialized knowledge, such as program analysis and invariant generation. To address this, researchers have begun to explore ways of enhancing LLMs with domain-specific guidance~\cite{zeng2023evaluating}. 

% In our study, we explored two different approaches to provide domain knowledge for assisting LLMs in generating invariants. 
% The first approach involved providing a set of general instructions (GIs) to the LLMs, instructing how to approach the problem of generating invariants. 
% The second approach consisted of breaking the problem down into smaller sub-problems, then combining the resulting partial solution invariants to formulate the final invariant. 
% We will elaborate on the details of these two approaches in the following sections.

In this study, we are motivated by the need to enhance LLMs' effectiveness in this domain by investigating how the method of providing domain knowledge influences their performance. Specifically, we intend to compare two strategies for guiding LLMs:  (1) supplying General Instructions (GIs) that guide how to approach invariant generation, and (2) decomposing the problem specification into smaller sub-tasks and combining the associated partial invariants. 

% \saikat{The above paragraph does not really say motivation, it is merely conveying what you did. Please rewrite this with the {\bf motivation}.}







\textbf{\paragraph{Approach 1:} General Instructions (GIs)} 
Our first approach in helping LLM with domain knowledge is to provide some general instructions as described in~\Cref{ssec: GI}.
% We designed these instruction to describe the invariant synthesis problem to the LLM. 
% \saikat{Describe individual }


\experiment 
For this experiment, we prompted the aforementioned LLMs with GIs to generate loop invariants. To setup the models, for Llama 3.1, we used Google Colab with an A100 GPU, equipped with 83GB of RAM and 40GB of GPU memory. For GPT-4 and Mistral-large, we accessed their official APIs. 
% To assess the initial producibility of the models, we selected a sample of 30 problems from the dataset. 
Initially, we randomly selected 30 problems and analyzed all three LLMs to understand if they are even capable of generating invariants. 
We evaluated the models based on their ability to follow instructions, produce parsable responses, and generate syntactically correct invariants. 
After analyzing the invariant generation capabilities of the models, we compared their performance of generating invariants with and without GIs on the complete benchmark dataset. 
% In this study, an invariant is considered successful if it passes the verification check performed by the verifier \textit{lig-verify} .

\resultsec 
% Table \ref{tab: GIcomparision} summarizes the experimental findings on the LLMs' ability to generate invariants from instructions.  For the sample 30 problems, all three LLMs generated some responses, regardless of whether those responses contains to expected invariant or not. We found that llama 3.1, couldn't completely follow the instruction of the output template (as mentioned in figure \ref{fig:prompt_gi}). We observe that the responses of Llama 3.1 contain some explanations inside the invariant in most of the cases, in several instances, it encountered issues with imbalanced brackets and tags. Additionally, some invariants were syntactically incorrect and our invariant extractor tool couldn't extract any complete invariant from these responses. In case of Mistral-large model, among 30, 25 responses followed the guiding output template, and 3 responses contained imbalanced tags and brackets in between the invariant code body which were marked as syntactically incorrect. In case of GPT-4o, all the responses were following the provided output template, the invariants were successfully extracted by the tool, and those were syntactically correct.          
Table \ref{tab: GIcomparision} summarizes the experimental findings on the LLMs' ability to generate invariants from instructions.  
For the sample 30 problems, all three LLMs generated some responses, regardless of whether those responses contains to expected invariant or not.  
We observe that the responses of Llama 3.1 mostly contains natural language description of the problem it is supposed to solve -- acting more like an helper to the developer who is writing the invariant. 
None of the generated responses by Llama-3.1 followed the output template we instructed in the prompt
As such, our automated invariant extraction tool is not able to extract {\em any} invariant for further verification and evaluation. 
There are couple of instances in Llama-3.1 responses, where our best effort heuristic response parser extracted an invariant -- almost all of those contained syntactic error, mostly related to imbalanced parentheses. 
Mistral-large responses were much better, where 25 solutions followed the output template and 22 among them were syntactically correct. 
All the responses from GPT-4o were correctly followed the output template and we did not encounter any syntax error while processing any of automatically extracted invariants from these responses. 
\lessons{GPT-4o and Mistral-large successfully generated loop invariants based on the given instructions, whereas Llama 3.1 (8B), under the specified setup, failed to produce useful responses relevant to our study.}


% Among the presented findings in the table, most of the LLMs rarely follow all the instructions, rather, they try to make use of some of the instructions and do not cross-check generated results with the prompted instructions. 
% Also, in many cases, generated invariants were not syntactically correct. 
% Also, some LLMs generate invariants, which were difficult to extract for the machine from their unstructured text responses. 
% Further analysis of the generated invariants from the study indicates that most of the invariants are incorrect and do not satisfy verification conditions. 
% \saikat{All these results are very anecdotal. There is no particular evidence that backs up these claims. Please add tables and numbers, so that it doesn't sound like we are making this stuff up. }

\begin{table}[!t]
    \centering
    \caption{Performance comparison of LLM models general instructions.}
    \footnotesize
    % \resizebox{\linewidth}{!}
    { % This ensures the table fits within the column
        % \begin{tabular}{|p{0.2\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|p{0.1\linewidth}|}
        %     \hline
        %     \multirow{2}{*}{\textbf{LLM Model}} & \multicolumn{3}{|c|}{\textbf{With General Instruction}} & \multicolumn{3}{|c|}{\textbf{Without General Instruction}} \\
        %     \cline{2-7}            
        %     & $k=10$ & $k=30$ & $k=50$ & $k=10$ & $k=30$ & $k=50$ \\ \hline 
        %     GPT-4o & 27\% & 41\% & 49\% & 19\% & 32\% & 40\% \\ \hline  
        %     Mistral-large & 21\% & 27\% & 31\% & 13\% & 18\% & 21\% \\ \hline
        % \end{tabular}
        \begin{tabular}{c|c|c|c|c|c|c}
        & \multicolumn{6}{c}{\textbf{\% of problems solved in k generated responses}}\bigstrut \\
        \cline{2-7}
        \multirow{2}{*}{\textbf{LLM}} & \multicolumn{3}{c|}{\textbf{Without GI}} & \multicolumn{3}{c}{\textbf{With GI}}\bigstrut[t] \\
        & $k=10$ & $k=30$ & $k=50$ & $k=10$ & $k=30$ & $k=50$ \bigstrut[b] \\
        \hlineB{2}
        Mistral-large & 13 & 18 & 21 & 21 & 27 & 31  \bigstrut\\ 
        GPT-4o & 19 & 32 & 40 & 27 & 41 & 49 \bigstrut \\
        \hlineB{2}
        \end{tabular}
    }
    \label{tab:GI_performance}
\end{table}
% Under the same setup, Mistral-large achieved a highest success rate of 31\%. Notably, 
Given the poor performance of Llama-3.1, we restrict our further investigation to only Mistral-large and GPT-4o.
To assess the effectiveness of the General Instructions (GIs), we tasked GPT-4 and Mistral-large with generating 50 invariants ($k=50$) for each of the problems using the GI prompt (\Cref{fig:prompt_gi}). 
As shown in ~\Cref{tab: GIcomparision}, both Mistral-large and GPT-4o are benefited from the general instructions. 
GPT-4 generates at least one successful invariant for 49\% (103 out of 210) of the problems when we put the GIs in the prompt, compared to 40\% without the instructions.
We also observe similar impact of GIs in Mistral-large. 
Note that we do not intend to compare performance across different LLMs, our goal is to empirically identify the impact of the GIs while generating loop invariants.
Experimentally, we observe both models demonstrated a comparatively higher success rate when using the GI-based prompts than when using prompts without GIs. 
This highlights the positive impact of the general instruction set on the models' performance in generating valid invariants.   
\lessons{Both Mistral-large and GPT-4o generated more successful invariants with the instructions}
% On the other hand, asking for a single invariant for a sygus-like problem and evaluating the LLM model based on that is always harsh. In this regard,  we asked the Mistral-large, GPT-3.5, and GPT-4o models to produce thirty ($ k = 50$) invariants and found 12\%, 12\%, and 28\% of the problem can be satisfied by at least one invariant respectively.                

% \begin{table*} [!t]
% \caption{Study on LLM's Invariant Generation using GIs {\todo{See TODO 4-3}}}
%     \centering
%     \begin{tabular}
%       {|p{.16\linewidth}|p{.16\linewidth}|p{.16\linewidth}|p{.18\linewidth}|p{.14\linewidth}|} \hline
%          \textbf{LLM Model}&  \textbf{Produce Invariants?} &  \textbf{Follow instructions?}&  \textbf{Syntactically correct?}&  \textbf{Easy to Extract Invariants?}\\ \hline
%          Llama 3 8b&  Yes&  Rarely &  Rarely &  No\\ \hline
%          llama 3.1 8b&  Yes&  Rarely &  Rarely &  No\\ \hline
%          Mistral-large &  Yes&  Rarely &  Rarely &  Rarely \\ \hline
%          GPT-3.5&  Yes&  Yes&  Yes&  Yes\\ \hline
%          GPT-4o&  Yes&  Yes&  Yes&  Yes\\ \hline
%     \end{tabular}    
%     \label{tab: GIcomparision}
% \end{table*}

% \lessons{GPT-4o and Mistral-large were able to generate loop invariants from the general instructions for a low-level program specification} 

% \lessons{Llama 3.1(8b), in the specified setup, was unable to generate invariants following the provided specifications}

% \lessons{LLMs may not verify their responses with the prompting conditions \saikat{How do you come to this conclusion?}}

% \lessons{GPT-4o performs better in following the instructions \saikat{Again, numbers?}}


% \lessons{GPT-4o achieves higher success rate of 49\% in generating successful invariants following the provided instructions}

 \begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/partial_prompt.pdf}
    \caption{Prompt template to utilize partial invariant synthesize }
    \label{fig:partial-prompt}
\end{figure}

\textbf{\paragraph{Approach 2:} Invariant problem partitioning}

% From the result of the previous approach, we identified that the general instructions got the maximum success of 49\%, highlighting the potential for exploring more comprehensive approaches. 

% So, we tried another approach to help the LLMs in generating invariants. 
% To alleviate the issue \saikat{which issue?}, we aim at helping LLM by partitioning the problem into smaller sub-problems and then combining the partial solutions to produce the final invariant. 
% As we know, a sysgus loop invariant problem needs to be satisfied with four conditions -  \saikat{Would be better if expressed as equations}

% Considering the nature of problems in our dataset, we observe that each of the problem's verification is composed of four underlying verification conditions. The conditions are -  

% \item pre-function implies to post-function \label{c1} 
    % \item pre-function implies to invariant-function \label{c2}
    % \item (transition-function and invariant-function) implies transition-function  \label{c3}
    % \item invariant-function implies to post-function \label{c4}
 A successful inductive loop invariant ($invF$), with precondition ($preF$), postcondition ($postF$) and loop body ($transF$) must satisfy the following three verification conditions simultaneously (see \cref{subsection:li} for details) 
\begin{enumerate} \label{sygus-conditions}
    % \item $preF(x,...) \Rightarrow postF(x,...)$ \label{c1} 
    \item $preF(x,...) \Rightarrow invF(x,...)$  \label{c2}  
    \item $ (tranF(x,...) \wedge invF(x,...)) \Rightarrow invF(x!,...)$ \label{c3}
    \item $invF(x,...) \Rightarrow postF(x,...)$ \label{c4}    
\end{enumerate}

Having such a natural composition of subproblems, we are interested in approaching the problem in a divide-and-conquer fashion. 
We prompted the LLMs separately for each invariant-related condition, instructing it to generate a set of invariants that satisfy the corresponding condition. 
After generating invariants for each of the conditions, we then asked the LLM to integrate them into single composed invariants, capable of satisfying all three conditions.

 % We aimed to check the LLM's ability of generating invariants with simplified conditions and then combine these invariants to satisfy the complete program.
 
 % Three of the above conditions (\ref{c2}, \ref{c3}, \and \ref{c4}) are directly related to invariants. A loop invariant is a logical expression that must satisfy all four conditions simultaneously. Dividing the invariant-generation process into separate satisfiability conditions may help LLMs better understand the problem domain and handle simpler logical satisfiability problems more effectively. This experiment aimed to simplify the LLM’s task by breaking it down into smaller, more manageable conditions and improving the success rate.
 
% In this approach, we prompted the LLMs separately for each invariant-related conditions, instructing it to generate a set of invariants that satisfy the corresponding condition. After generating invariants for each of the conditions, we then asked the LLM to integrate them into single composed invariants, capable of satisfying all four conditions.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/combined.pdf}
    \caption{Prompt for combining partial invariants}
    \label{fig:combined_prompt}
\end{figure}

\experiment To set this experiment, we designed a new prompt (figure \ref{fig:partial-prompt}) for a single condition above, omitting the details of unrelated things. 
For example, Equation \ref{c2} requires precondition and invariant only; we omit details related to the loop body and postcondition from this prompt.   
In this way, we are relaxing the problem into three easier subproblems. We call these three prompts $\mathcal{P}_{pre}$, $\mathcal{P}_{trans}$, and $\mathcal{P}_{post}$ (referred collectively as $\mathcal{P}_{partial}$), respectively each corresponding to only the conditions \ref{c2}, \ref{c3}, and \ref{c4}, respectively. 
After getting the invariants ($\mathcal{I}_{conditional}$) for each condition, we asked LLMs to combine them to generate the final invariants($\mathcal{I}_{final}$) -- we call this prompt $\mathcal{P}_{full}$. 
Concretely, we instructed the LLMs to generate ten $\mathcal{I}_{conditional}$s ($k=10$) independently using each of $\mathcal{P}_{pre}$, $\mathcal{P}_{trans}$, and $\mathcal{P}_{post}$. 
We then test the generated $\mathcal{I}_{conditional}$ using a modified version of the verifier, which only checks satisfiability of the corresponding condition.
Thus, for each problem, we have thirty $\mathcal{I}_{conditional}$s and corresponding verification results.
Next, we create the $\mathcal{P}_{full}$ (see \Cref{fig:combined_prompt} as an illustration) with all of these $\mathcal{I}_{conditional}$s and corresponding results and instruct LLMs to generate fifty ($k=50$) $\mathcal{I}_{final}$. 

Our rationale behind showing the failed candidate from an individual trial in addition to the successful ones is that we want to demonstrate what had gone wrong (since we are also presenting the partial verification results), and help LLMs avoid certain mistakes. 

% Since the final verification condition is the conjunction of all three conditions, one may argue that
% Next, we prompted the LLMs to generate fifty ($k=50$) combined invariants by utilizing generated thirty candidate invariants in earlier step and their verification outcomes. 
 % The experiment was conducted with GPT-4o because the other models were comparatively less performing to follow the given instructions. We asked the LLM to generate several invariants (k=4) for each condition. Each of the invariants was tested with the verifier, and with the verification results, we prompted again the LLM to generate several combined invariants that satisfy all the conditions.     



% We randomly selected 30 SyGus problems from the dataset to conduct this experiment. 
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figures/partial-inv-res-patterns.pdf}
    \caption{Success rate with partitioning invariant problem}
    \label{fig:partial-inv-res}
\end{figure}

% Figure \ref{fig:partial-inv-res} provides a summarized figure of the findings. 
% Across both the LLMs, we observed that simpler conditions such as equation \ref{c2} and \ref{c4} had higher success rates, with 60\% and 59\% of problems successfully verified, respectively. In contrast, condition \ref{c3}, which is more complex, achieved a lower success rate of 41\%.

\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/venn_gpt4.pdf}
        \caption{GPT-4 generated invariants}
        \label{fig:gpt-4-venn}
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\linewidth}
        \includegraphics[width=\linewidth]{figures/venn_mistral.pdf}
        \caption{Mistral generated invariants}
        \label{fig:mistral-venn}
    \end{subfigure}%
    \caption{Comparative numbers of sub-problems where LLMs generated correct invariants.}
    \label{fig:venn}
\end{figure}

\resultsec Figure \ref{fig:partial-inv-res} provides a summarized figure of the findings. 
Across both the LLMs, we observed that simpler conditions such as equation \ref{c2} and equation \ref{c4} had higher success rates than the more complex condition (\ie equation \ref{c3}). 
For example, for conditions \ref{c2} and \ref{c4}, GPT-4o's success rate is 45\% and 40\%, respectively, while for condition \ref{c3}, it is merely 15\%. 

% When combined with the $\mathcal{P}_{full}$, the performance is similar (or slightly better) to the performance in condition \ref{c3}. 

When combined with the $\mathcal{P}_{full}$, the performance is lower than the performance on individual conditions. To understand the results better, we analyzed the subset of problems where LLMs could generate invariants satisfying each of these conditions. 
\Cref{fig:venn} shows the intersection of problems where LLM could generate a successful solution with the partial prompts and full prompt. 

In the case of GPT-4, there are 26 problems, where LLMs generate correct solution for each of the three $\mathcal{P}_{partial}$s. However, only 15 of those problems were solved with the $\mathcal{P}_{full}$. For Mistral, 16 problems had solutions satisfying all three prompts separately, but when combined, only 9 problems were solved. 

We analyzed the generated invariants with $\mathcal{P}_{full}$ and $\mathcal{P}_{partial}$s to understand why LLM failed to produce satisfying $\mathcal{I}_{final}$, even though they found satisfying $\mathcal{I}_{conditional}$ for all three conditions.   

% Due to the unpredictable behavior of LLMs \cite{huang2024survey}, understanding why the integration of $\mathcal{I}_{conditional}$s fails remains unclear. Our findings suggest that integrating logical expressions (\ie $\mathcal{I}{conditional}$) poses computational challenges, potentially being NP-hard \todo{ref}. The generation of valid $\mathcal{I}_{conditional}$s was constrained to a fixed quantity, with no assurance that a valid $\mathcal{I}_{final}$ could emerge from any combination of them. Consequently, instructing the LLM to generate $\mathcal{I}_{final}$s from the given valid $\mathcal{I}_{conditional}$s may inadvertently restrict its search space, potentially leading to unsuccessful $\mathcal{I}_{final}$ generations.

We conjecture that integrating logical expressions (\ie $\mathcal{I}_{conditional}$) poses computational challenges, potentially being undecidable ~\cite{si2018learning}. The generation of valid $\mathcal{I}_{conditional}$s was constrained to a fixed quantity, with no assurance that a valid $\mathcal{I}_{final}$ could emerge from any combination of them. In addition, we anecdotally tested ten (10) problems with manually constructed $\mathcal{P}_{full}$ containing at least one ground truth invariant. Analyzing the generated $\mathcal{I}_{final}$s ($k=50$), we found that none of the generated invariants matched the input ground truth invariant, suggesting that LLMs struggle to infer correct invariants even when provided with strong supporting examples.

   

% \todo{finish this paragraph}



% Consequently, instructing the LLM to generate $\mathcal{I}_{final}$s from the given valid $\mathcal{I}_{conditional}$s may inadvertently restrict its search space, potentially leading to unsuccessful $\mathcal{I}_{final}$ generations. 


% Interestingly, in GPT-4, there are four problems that were solved exclusively $\mathcal{P}_{full}$, even though there were no correct solution satisfying any of those three conditions when asked with $\mathcal{P}_{partial}$s. 

% From the venn diagrams in \Cref{fig:venn}, it is evident that the problems that are solved by the combined prompt is not strict subset or superset of the problems solved with any of the $\mathcal{P}_{pre}$, $\mathcal{P}_{trans}$, and $\mathcal{P}_{post}$. 

% Having observed the result, we conjecture that dividing the loop invariant synthesis problem into subproblems and then combining their solutions, results in a low success rate, reaching a maximum of only 8\% in our experimental setup.

% \saikat{To be finished after getting the venn diagrams from }


\lessons{Dividing the loop invariant synthesis problem into subproblems and then combining their solutions, results in a low success rate, reaching a maximum of only 8\% in our experimental setup.}

% Finally, combining the partial invariants using the LLM resulted in a 39\% success rate in verification. 
% Comparatively, Mistral-large performed worse than GPT-4o across all invariant generation tasks.





% \lessons{Dividing the loop invariant satisfaction problem into sub-problems is helpful to guide LLM in producing more successful invariants for sub-problems \saikat{What is the evidence behind this lesson?}}

% \lessons{ Dividing the problem into sub-conditions achieved a maximum success rate of 39\%, which is comparatively lower than the success rate obtained with the general instructions (49\%)}

% \lessons{LLMs were able to generate 10\% successful combined invariants using partitioned invariant problem analysis}

% \RS{1}{The results}

% \textbf{\paragraph{Discussion:} Findings of RQ1.1}

% We constructed domain knowledge for LLM with strategies - GIs-based and divide-and-conquer-based. Experiments suggest that LLM have a higher success rate with GIs (49\%) compared to baseline(40\%) and divide-and-conquer-based (8\%).   

% We conducted experiments to enhance Large Language Models (LLMs) with domain knowledge, employing two strategies: providing general instructions on invariant inference and partitioning the problem into sub-problems. Our experimental results were promising when we included general instructions in the prompts, showing a significant improvement compared to prompts without specific instructions. Conversely, the approach of breaking the problem into sub-problems did not yield favorable results. In fact, our findings indicated that problem partitioning performed worse than the base prompt with no instructions.
  

% The experiment on \textit{\textbf{RQ1.1}} shows that with the different types of instructions, LLMs can generate invariants for low-level program specifications,  . But in general, LLMs are not following all the instructions, rather, they try to make use of some of the instructions and do not cross-check generated results with the prompted instructions. Also, in many cases, generated invariants were not syntactically correct. On the other hand, LLM can generate successful invariants with comparatively smaller conditions. However, LLM faces difficulties in combining the partial invariants to generate the final invariant. Compared to other available LLMs, GPT-4o is more likely to follow the instructions and generate invariants that satisfy the verification conditions. \saikat{This paragraph sounds like a paraphrase of the lessons state above. What is the point?}


% We experimented the ability of LLMs in synthesizing loop in-
% variant with the help of the problem’s domain knowledge. With
% a generalized invariant synthesizing instruction set, the best per-
% forming LLM achieves 49\% success rate. On the other hand, with
% partitioning the bigger problem into meaningful subproblems, iden-
% tifying solutions to subproblems, and combining solutions from
% subproblems achieves a success rate of up to 39% for GPT-4o. Over-
% all, these settings of the problem’s domain knowledge can’t help
% LLM to achieve a higher success in loop invariant generation.

% We experimented with the ability of LLMs to synthesize loop invariants using the problem's domain knowledge, which was constructed with two components: 1) our collected invariant generation instructions and 2) partitioning the problem into concise subproblems. When comparing the results of plain prompts, instructions-based prompts, and the partitioning approach, our proposed instruction-based prompt achieved the highest success rate of 49\%. However, it is important to note that our method of partitioning the problem did not surpass the success rate of the baseline plain prompt approach.           


\subsubsection{[RQ1.2]} Can LLMs generate loop invariants by learning from similar examples?

\motivation
% In the previous experiment, we found that domain knowledge is helpful for LLMs in generating loop invariants \saikat{It is not evident from the previous section comain knowledge is actually helpful.}, but the issue is that for LLMs, it is difficult to resolve all the conditions \saikat{What does this sentence mean? -- doesn't make sense}. 
% On the other hand, existing studies show that LLMs are good at learning from examples. Few-shot learning is a popular approach to help LLMs learn from examples. 
% To alleviate the issue \saikat{Again, what ``issue'' are you alleviating?}, we help LLM by providing similar examples to the problem. 

In the previous section, we examined how domain knowledge influences the generation of loop invariants by LLMs, achieving a success rate of up to 49\%. While this result demonstrates potential, it underscores the need for further enhancement. Prior research, such as \cite{brown2020language, yoshida2024impact, misu2024towards}, has shown that LLMs are particularly adept at learning from examples. Few-shot learning, a widely used technique, can effectively harness this capability by providing the model with a set of illustrative examples, specifically, in this study, we refer to the problems in our benchmark that include at least one solution invariant. To investigate whether LLMs can improve their performance in loop invariant generation through example-based learning, we experimented with this study in two approaches.

% In the first approach, we examined the impact of examples using few-shot learning with examples, selected by several example-finding algorithms \Cref{ssec:algo}, referred to as similarity finding algorithms. These algorithms help retrieve the most similar existing problems from our dataset. We identified two similarity finding algorithms: 1) Semantic similarity, powered by a BERT-based semantic text similarity algorithm, and 2) Syntactic similarity, developed using an AST tree-based syntactic similarity finding algorithm. We discussed the algorithms in Section \ref{ssec:algo}.

In the first approach, we examined the impact of examples using few-shot learning with examples, discovered by two example-finding algorithms, as we mentioned in ~\Cref{ssec: algo}. 
In the second approach, we conducted the few-shot learning experiment utilizing different types of examples (discussed in ~\Cref{ssec: examples}). 

% : 1) Positive examples and 2) Negative examples.  Positive examples are those that satisfy all verification conditions, guiding the LLM to follow patterns that lead to successful solutions. In contrast, negative examples do not satisfy all verification conditions and serve to help the LLM avoid potential patterns that result in unsuccessful solutions. As researchers \cite{yoshida2024impact, li2024turning} have demonstrated that LLMs can learn from negative examples to address negative outcomes, we aimed to incorporate negative examples to decrease the likelihood of generating negative invariants in the responses.


\textbf{\paragraph{Approach 1:} Impact of similarity algorithms in few-shot example discovery} 
% \saikat{Wouldn't it be better if you showed this as approach1, and current approach 1 as approach 2?}
% Selecting the appropriate examples to form a few-shot prompt can have a significant impact.  
% However, a closer look at the examples indicates that the similarity between the query and examples provided in the few-shot can play a vital role in generating successful invariants. 

% \saikat{A reader would have no idea what any of these similarity metrics mean? \S3.3 gives a mere overview, we may need to go in deep how we calculated these similarities?}

 
% We also observed that the BART-based similarity, considered in the earlier experiment, takes semantic similarity into account. 
% On the other hand, syntactic similarity can also be important, as problems with similar types of operations seem likely to have similar invariants. 

In ~\Cref{ssec: algo}, we analyzed the distinguishing characteristics of the examples retrieved by the similarity-based algorithms for the query problem. This experiment aims to evaluate the extent to which each algorithm supports the large language model (LLM) in generating a valid invariant for the given problem.

\experiment
% To test the impact of similarity measures in the few-shot prompting, we prepared the prompt with the similar problems and their associated successful invariant retrieved by each of the similarity algorithms. 
% % \saikat{In the previous experiment, did you also use 2-shot prompting? If yes, why 2, not other numbers (an ablation on a number of few shot examples, perhaps). If not, how would you explain and defend this design choice?}

% We examined the performances of LLMs for three different sample sizes ($k=10, 30, 50$) to identify the patterns in success. 

% % \saikat{Why are the {\tt k}'s inconsistent across different experiments? You need to clearly explain and defend this design choice. }

We adopt the prompt setup illustrated in ~\Cref{fig:few-shot-template} for this experiment. We apply the algorithms $\mathcal{S}_{semantic}$ and $\mathcal{S}_{syntactic}$ to retrieve a small set of positive examples, $\mathcal{EX}_{P}$ (with $n=2$) to populate the few-shot prompts. Since the objective of this experiment is to evaluate the performance of the similarity algorithms, we intentionally omit discussion of the rationale behind the types of examples (~\Cref{ssec: examples}) and their quantity, assuming that any such effects are consistent across algorithms. To assess the performance of the LLMs, we evaluate the generated results using sample sizes of $k = 10$, $30$, \& $50$.

\resultsec

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/fewshot_baseline.pdf}

%     \caption{Success rate Comparison of different prompts }
%     % \saikat{The texts in the figure are very hard to read.}
%     \label{fig: Comp_similariyP}
% \end{figure}


\begin{table}[!t]
    \centering
    \caption{Performance comparison of LLM models with General Instructions.}
    \footnotesize
    % \resizebox{\linewidth}{!}
    { % This ensures the table fits within the column
       
        \begin{tabular}{c|c|c|c|c|c|c}
        & \multicolumn{6}{c}{\textbf{\% of problems solved in k generated responses}}\bigstrut \\
        \cline{2-7}
        \multirow{2}{*}{\textbf{LLM}} & \multicolumn{3}{c|}{\textbf{Few-shot with $\mathcal{S}_{semantic}$}} & \multicolumn{3}{c}{\textbf{{Few-shot with $\mathcal{S}_{syntactic}$}}}\bigstrut[t] \\
        & $k=10$ & $k=30$ & $k=50$ & $k=10$ & $k=30$ & $k=50$ \bigstrut[b] \\
        \hlineB{2}
        Mistral-large & 29 & 42 & 66 & 53 & 67 & 73  \bigstrut\\ 
        GPT-4o & 43 & 57 & 72 & 61 & 72 & 76 \bigstrut \\
        \hlineB{2}
        \end{tabular}
    }
    \label{tab:fewshot_performance}
\end{table}


% \begin{table*}[!t]
%     \centering
%     \caption{Performance comparison of LLM with few shot prompts}
%     \resizebox{0.9\linewidth}{!}{ % This ensures the table fits within the column
%         \begin{tabular}{|p{0.2\linewidth}|p{0.07\linewidth}|p{0.07\linewidth}|p{0.07\linewidth}|p{0.07\linewidth}|p{0.07\linewidth}|p{0.07\linewidth}|p{0.07\linewidth}|p{0.07\linewidth}|p{0.07\linewidth}|}

%             \hline
%             \multirow{2}{*}{\textbf{LLM Model}} & \multicolumn{3}{|c|}{\textbf{General Instruction}} & \multicolumn{3}{|c|}{\textbf{Few-Shot with semantic similarity}} & \multicolumn{3}{|c|}{\textbf{Few-Shot with syntactic similarity}} \\
%             \cline{2-10}            
%             & $k=10$ & $k=30$ & $k=50$ & $k=10$ & $k=30$ & $k=50$ & $k=10$ & $k=30$ & $k=50$\\ \hline 
%             GPT-4o & 27\% & 41\% & \textbf{49\%} & 43\% & 57\% & \textbf{72\%} & 61\% & 72\% & \textbf{76\%} \\ \hline  
%             Mistral-large & 21\% & 27\% & 31\% & 29\% & 42\% & \textbf{66\%} & 53\% & 67\% & \textbf{73\%} \\ \hline
%         \end{tabular}
%     }    
%     \label{tab:fewshot_performance}
% \end{table*}


Table \ref{tab:fewshot_performance} presents the comparative analysis of the $\mathcal{S}_{semantic}$ and $\mathcal{S}_{syntactic}$ similarity-based selection strategies for few-shot prompting, evaluated with the GPT-4o and Mistral-large models. For the sample size, $k=10$, the $\mathcal{S}_{syntactic}$ yielded a higher success rate (61\% for GPT-4o and 53\% for Mistral-large) compared to the $\mathcal{S}_{semantic}$ (43\% and 31\% respectively). With both models, $\mathcal{S}_{syntactic}$ continues to show better performance with the larger batch sizes, $k=30$ and $k=50$. Notably, for $k=50$, $\mathcal{S}_{syntactic}$ achieved the highest success rate of 76\% with GPT-4o, while $\mathcal{S}_{semantic}$ produced a slightly lower success rate of 72\%. These results suggest that as the sample size increases, the difference in performance between the two similarity measures diminishes. Furthermore, both similarity-based few-shot prompting strategies substantially outperform the instruction-only baseline.




% \saikat{This is the fist result I see which is convincing}

% \lessons{The examples in few-shot are more useful for invariant generation}
\lessons{The syntactic similarity measure yielded up to 76\% success rate for the sample size $k=50$ with few-shot learning}
\lessons{With GPT-4o, for the lower number of sample size ~\ie $k=10$, the performance difference for the algorithms is 18\%, while with a higher sample size $k=50$, the performance difference is as small as 4\%}


% \textbf{\paragraph{Analysis:} Impact of the similarity in the few-show prompt \saikat{What does that even mean?}}

% We have conducted an extensive study on the impact of few-shot example selection to verify the contribution of similarity. \saikat{What do you mean by ``extensive study''? What are the results that you presented before?}
% The study indicates that the examples in the few-shot are more useful for invariant generation. \saikat{I thought we already established that few-show examples are useful}

% \textbf{ \paragraph{ Analysis:} Impact of the similarity of the examples in few-shot prompt}
% From the previous experiment, we can conclude that the syntactic similarity works fine to pick the right example based on the performance gain. To further analyze the impact of selecting the most similar example in few-shot, we tested LLMs with examples of different orders of similarities. \todo{update} 

% \experiment
% We selected 30 random problems from the dataset and prompted GPT-4o to produce loop invariants. For each of the problems, we identified the top ten similar problems from our dataset with having at least one ground truth successful invariant using both of the similarity algorithms. In the first iteration, prompts were generated with the first two similar problems and corresponding invariants. In the second iteration, the prompt was composed of the third and fourth similar problems, and so on up to five iterations. We have analyzed the $pass@k$ for each of the iterations. We followed the algorithm presented by Chen et al. \cite{chen2021evaluating} to calculate the $pass@k$.    


% \resultsec

% The results of the experiment are presented in Figure \ref{fig: rank_example}, demonstrating the impact of examples based on their similarity in few-shot prompting. 
% We observe that for both algorithms, the top-ranked or most similar examples help the LLM generate more successful invariants. 
% For the syntactic similarity example set, the pass rate is 45\% when we composed the few-shot with the first two most similar examples, the success rate becomes 34\% for the few-shot generated with the third and fourth similar examples. The performance is linearly declining with the few-shots composed of lower ranked examples. Similarly, in the case of semantic similarity,  we observed the tendency to perform better with higher-ranked examples. We noticed in the fourth iteration, the performance of LLM is better than the second and third iterations. We conducted some manual analysis to understand the cause behind this. We found that, for the semantic similarity algorithm, some examples that rank higher in syntactic similarity appear in lower ranks, potentially affecting the performance. 
% Table \ref{tab:similarity_ranks} represents the top 10 corresponding similar problems captured by each of the similarity methods for the query problems with ID 203 and 301. Here ID is the problem's representing identity in our database. We observed that the problem with id 438 ranked second for query problem 203 in the syntactic similarity Method, on the other hand, it appeared at rank four with the semantic similarity method. Similarly, for the query problem 301, 914 ranked third and eighth correspondingly.  
% % \saikat{What is a reader supposed to understand from the above sentence?}. 
% Considering the impactful examples in few-shot, which appear in the higher ranks in syntactic similarity algorithm but comparatively lower ranks in semantic similarity search, are more likely to key for the better performance of the semantic similarity algorithm in later iterations. 


% \begin{figure} [!t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/similarity_ex_pass@5.pdf}
%     \caption{Performance analysis on the rank of examples in few-shot prompts}
%     \label{fig: rank_example}
% \end{figure}


% \begin{table}[!t]
%     \caption{Comparison of problem IDs captured by similarity methods.}
%     % \saikat{This table does not objectively convey any message.}}
%     \centering
%     \renewcommand{\arraystretch}{1.5} % Adjust row height
%     \begin{tabular}{|>{\centering\arraybackslash}m{1.2cm}|>{\centering\arraybackslash}m{1.4cm}|>{\centering\arraybackslash}m{4.7cm}|}
%         \hline
%         \textbf{Query Problem Id} & \textbf{Similarity Method} & \textbf{Similar Problem IDs- Sorted on Rank} \\ 
%         \hline
%         \multirow{2}{*}{203} & Syntactic & 100, \underline{438},324,98,447,502,837,466,625,573 \\ 
%         \cline{2-3}
%         & Semantic & 696,275,98,\underline{438},447,502,837,811,16,398 \\ 
%         \hline
%         \multirow{2}{*}{301} & Syntactic & 213, 121, \underline{914}, 322, 6, 274, 918, 818, 635, 190 \\ 
%         \cline{2-3}
%         & Semantic & 412, 507, 834, 274, 121, 213, \underline{914}, 888, 322, 912 \\ 
%         \hline
%     \end{tabular}
    
    
%     \label{tab:similarity_ranks}
% \end{table}



% \begin{table}[t]
%     \caption{Comparison of Syntactic and Semantic Measures}
%     \centering
%     \renewcommand{\arraystretch}{1.5} % Adjust row height
%     \begin{tabular}{|>{\centering\arraybackslash}m{1cm}|>{\centering\arraybackslash}m{1.1 cm}|>{\centering\arraybackslash}m{1 cm}|>{\centering\arraybackslash}m{1cm}|>{\centering\arraybackslash}m{1.1 cm}|>{\centering\arraybackslash}m{1cm}|}
%     \hline
%         \multicolumn{3}{|c|}{\textbf{Syntactic (Distance)}} & \multicolumn{3}{c|}{\textbf{Semantic (Similarity)}} \\ \hline
%         \textbf{Mean} & \textbf{Median} & \textbf{SD} & \textbf{Mean} & \textbf{Median} & \textbf{SD} \\ \hline
%         18.10 & 7.5 & 23.72 & 4.60 & 4.61 & 0.05 \\ \hline
%     \end{tabular}
    
%     \label{tab:similarity_stats}
% \end{table}



% \begin{table}[h]
%     \centering
%     \renewcommand{\arraystretch}{1.5} % Adjust row height
%     \begin{tabular}{|p{0.12\linewidth}|p{0.09\linewidth}|p{0.12\linewidth}|p{0.09\linewidth}|p{0.09\linewidth}|p{0.12\linewidth}|p{0.09\linewidth}|}
%     \hline
%     \textbf{Top N Examples} & \multicolumn{3}{c|}{\textbf{AST}}  & \multicolumn{3}{c|}{\textbf{BERT}} \\ \hline
%     & \textbf{Mean} & \textbf{Median} & \textbf{SD} & \textbf{Mean} & \textbf{Median} & \textbf{SD} \\ \hline
%     1  & 14.12 & 6.00 & 20.67 & 4.61 & 4.61 & 0.05 \\ \hline
%     2  & 17.66 & 7.50 & 23.80 & 4.60 & 4.61 & 0.05 \\ \hline
%     3  & 21.12 & 9.13 & 26.79 & 4.60 & 4.61 & 0.06 \\ \hline
%     4  & 24.16 & 11.00 & 29.45 & 4.60 & 4.61 & 0.07 \\ \hline
%     5  & 27.11 & 13.33 & 31.89 & 4.59 & 4.61 & 0.07 \\ \hline
%     6  & 29.84 & 15.00 & 34.06 & 4.59 & 4.61 & 0.08 \\ \hline
%     7  & 32.32 & 18.00 & 35.93 & 4.58 & 4.61 & 0.08 \\ \hline
%     8  & 34.58 & 20.00 & 37.62 & 4.58 & 4.61 & 0.09 \\ \hline
%     \end{tabular}
%     \caption{Comparison of AST and BERT Performance Across Top Examples}
%     \label{tab:similarity_stats2}
% \end{table}

% Table \ref{tab:similarity_stats} presents the statistical analysis of the similarity measurement algorithms, focusing on Syntactic (Distance) and Semantic (Similarity) metrics. The study is based on the first two examples, which played a key role in generating successful invariants, flexible with a value of k up to 50. From the data, it is evident that the BERT-based semantic similarity algorithm shows a very low standard deviation (0.05), suggesting that the algorithm struggles to distinguish between closer examples, producing very similar results even for items that may differ syntactically. The mean and median for the semantic similarity are also very close (4.60 and 4.61, respectively), reinforcing this consistency and lack of variability in the example finding. In contrast, the Tree-based distance calculation algorithm identifies dissimilarities between examples. With a higher mean of 18.10 and a much larger standard deviation (23.72), the tree-based algorithm demonstrates a much higher level of variability, indicating that it can differentiate between syntactically distinct items. 

% \lessons{Similarity of the example in the few-shot prompting is a useful metric \saikat{How do you learn this lesson after this RQ1.2?}}

% \lessons{With the most similar examples GPT-4o got success rate 45\%, and }


\textbf{\paragraph{Approach 2:} Few-shot learning with different types of examples}

\experiment
 
In the previous approach, we examined the impact of example selection based on similarity algorithms. In this approach, we shift our focus to the types of examples, as categorized in~\Cref{ssec: examples}. Using the verification outcomes of invariants, we constructed few-shot prompts (illustrated in~\Cref{fig:few-shot-template}) with three configurations: $\mathcal{EX}_{P}$ (positive examples), $\mathcal{EX}_{N}$ (negative examples), and $\mathcal{EX}_{Mix}$ (a combination of both). We adopted the same experimental setup as the previous approach, using examples retrieved via the $\mathcal{S}_{syntactic}$ algorithm, which previously demonstrated superior performance.



% were selected from different perspectives. As previously mentioned, we categorized examples based on the verification results of the generated invariants into two types: (1) Positive examples and (2) Negative examples. 
% Accordingly, we designed three different few-shot prompting strategies: 1) Few-shot (Positive): The prompt consists solely of positive examples . 2) Few-shot (Negative): The prompt consists solely of negative examples 3) Few-shot (Positive and Negative Mixed): The prompt includes a combination of both positive and negative examples. For selecting the examples, we considered the syntactic similarity algorithm, as its proven effectiveness in the previous section. 

% The experiment was conducted with Mistral-large, GPT-3.5, and GPT-4o. The generated invariants were tested with the verifier. 
% \saikat{Why do you keep repeating things that you have already said?}


\begin{table}[!t]
    \centering
    \caption{Study on LLM's Successful Invariant Generation with few-shot prompts: will be updated}
    \footnotesize {
        \begin{tabular}{c|c|c|c|c}
         & \multicolumn{4}{c}{\textbf{\% of problems solved in k generated responses}}\bigstrut \\
         \cline{2-5}
         \multirow{2}{*}{\textbf{LLM}} & \multirow{2}{*}{\textbf{Zero shot}} & \multicolumn{3}{c}{\textbf{Few-shot}}\bigstrut[t] 
         \\
         % \cline{3-5}
       &  & $\mathcal{EX}_{P}$ & $\mathcal{EX}_{N}$ & $\mathcal{EX}_{Mix}$
        \bigstrut[b] \\
        \hlineB{2}
        Mistral-large & 21\% & \textbf{73\%} & 23\% & 68\%  \bigstrut\\  
        % GPT-3.5&  13\% & \textbf{27\%} & 7\% & 13\% \\ \hline
        GPT-4o&  40\% & \textbf{76\%} & 34\% & 71\%  \bigstrut\\ 
         \hlineB{2}
    \end{tabular}
    }   
      
    \label{tab: few-shotComparison}
\end{table}

\resultsec  
  
Table \ref{tab: few-shotComparison} shows that both LLMs perform better when given only positive examples in the few-shot prompt. With $\mathcal{EX}_{P}$s, GPT-4o achieves a success rate of 76\%. In contrast, $\mathcal{EX}_{N}$s and  $\mathcal{EX}_{Mix}$ under the same setup yield lower success rates of 34\% and 61\%, respectively. We examined individual cases to understand how LLMs learn from examples. For example  a problem with the ground truth invariant {\texttt{(and (>= x 1) (<= x 101))}}, $\mathcal{EX}_{P}$ provided the invariant - {\texttt{(>= x 1))}} as example in the prompt, and  GPT-4o produced the invariant  {\texttt{(and (>= x 1) (<= x 101))}}, that is exactly same as the ground truth, on the other hand $\mathcal{EX}_{N}$ provided 
{\texttt{(and (<= x 11) (= y (- 10 x)}} as example, and GPT-4o produced {\texttt{(and (<= x 101) (> y (- 101 x)))}} as solution invariant.
This suggests that while negative examples help the model avoid certain incorrect patterns, they do not necessarily guide it toward the correct one due to the vast space of possible incorrect invariants. 

Furthermore, our results show that GPT-4o performs better in a zero-shot setting (40\%) than when prompted with $\mathcal{EX}_{N}$ examples (34\%). This finding further underscores the advantage of positive examples in effectively guiding the synthesis of correct invariants.



% \todo{add examples}

% \saikat{This result is great. In would've been better if you could show two examples where positive example helps. And also provide in-details argument saying why using negative example is not a that useful. (there are only a few potential correct solution, but infinite number of wrong solutions, \eg)}

\lessons{The few-shot (positive-only) approach achieved the highest success rate of 76\%, outperforming other example types discussed.}

% \lessons{In the few-shot example, the problem with satisfying invariants helps while unsatisfying invariants hinder the performance }

\textbf{\paragraph{Discussion:} Findings of RQ1.2}

% With extensive experiments on loop invariant generation problems by LLM, our study finds that few-shot example helps LLM better recognize the solution pattern. At the same time, for a sygus-like low-level program specification language, syntactic similarity for fetching examples is more successful than the semantic-based similarity example. 

Our finding from this study highlights two key points - 1) The similarity between the examples and the query problem significantly impacts performance. Our experiment showed that selecting the most syntactically similar examples led to a success rate of up to 76\%, compared to 72\% when using semantically similar examples. Additionally, the success rate difference became more significant as the number of sample generations decreased. 
2) LLMs learn invariant generation more effectively when provided with positive invariant examples. The few-shot setup with only positive examples achieved a 76\% success rate, outperforming approaches that used negative examples or a mix of positive and negative examples by a significant margin. 

% \todo{update}

\subsubsection{[RQ1.3]} Is the integration of domain knowledge and examples more useful for LLM to produce loop invariants?

\motivation
% As the instruction set \saikat{Do ``instructions'' really help? In RQ1.1, we have not seen a positive improvement after using instructions compared to not using instructions. In fact, you have not presented results without instructions.} and few-shot example, both can help LLMs generate loop invariants for low-level program specifications individually; we were interested in examining how LLMs respond if both are applied in the prompt. 
Based on the findings from RQ1.1 and RQ1.2, we determined that GIs and few-shot learning with positive examples are the most effective setups, respectively resulting in 49\% and 76\% success. In this research question, we aim to analyze the performance when both setups are combined.  


% \begin{table}[!t]
%     \centering
%     \caption{Performance comparison of LLMs with Combined Few-shot and Instruction-based prompts }
%     \resizebox{\linewidth}{!}{
%         \begin{tabular}{|p{0.4\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}|p{0.12\linewidth}|}

%             \hline
%             \multirow{2}{*}{\textbf{Prompt Choice}} & \multicolumn{3}{|c|}{\textbf{Success rate}}  \\
%             \cline{2-4}            
%             & $k=10$ & $k=30$ & $k=50$ \\ \hline 
%             Instruction only & 27\% & 41\% & \textbf{49\%} \\ \hline  
%             Few-shot only & \textbf{61\%} & \textbf{72\%} & \textbf{76\%} \\ \hline
%             Integrated Few-Shot with Instruction & 57\% & \textbf{73\%} & \textbf{78\%} \\ \hline
%         \end{tabular}
%      }
%     \label{tab: combined}
% \end{table}

\begin{table}[!t]
    
    \caption{Performance comparison of LLMs with Combined Few-shot and Instruction-based prompts}
    \centering
    \footnotesize{
    \begin{tabular}{p{.3\linewidth}|p{.15\linewidth}|p{.15\linewidth}|p{.15\linewidth}}
        & \multicolumn{3}{c}{\textbf{\% of problems solved in k generated responses}} \bigstrut \\
        % \cline{2-4}
        \textbf{Prompt Setup} & $k=10$ & $k=30$ & $k=50$ \bigstrut[b] \\
        \hlineB{2}
        Instruction only & 27\% & 41\% & \textbf{49\%} \bigstrut \\   
        Few-shot only & \textbf{61\%} & \textbf{72\%} & \textbf{76\%} \bigstrut\\ 
        Integrated Few-Shot with Instruction & 57\% & \textbf{73\%} & \textbf{78\%} \bigstrut\\         
        \hlineB{2}
    \end{tabular}  
    }
    \label{tab:combined}
\end{table}


\experiment
The experiment is designed by updating the prompts, appending the few-shot examples to the GIs within the prompt. We restricted the experiment to GPT-4o only, as it was the best-performing LLM model in RQ1.1 and RQ1.2.

\resultsec

The experiment combining instruction-based prompts with few-shot examples is summarized in Table \ref{tab: combined}. Excluding the cases where LLM's token limit was exceeded, the success rates of the generated invariants were 57\%, 73\%, and 78\% for $k = 10, 30, and 50$, respectively. The integrated approach yielded performance comparable to using only the few-shot positive examples, with a maximum improvement of just 2\% across all sample sizes. However, it is notable that 53\% of the prompts in the integrated setup exceeded the 8k token limit, resulting in failed requests.


% \saikat{What is the result only for those did not exceed the token limit? Compare the results for those are in-scope for RQ1.3, and then draw any conclusion}


% \begin{figure*} 
%     \centering
%   \subfloat[k=10\label{1a}]{%
%        \includegraphics[width=0.3\linewidth]{figures/pie_combined_10.png}}
%     \hfill
%   \subfloat[k=30\label{1b}]{%
%         \includegraphics[width=0.3\linewidth]{figures/pie_combined_30.png}}
%     \hfill
%   \subfloat[k=50\label{1c}]{%
%         \includegraphics[width=0.3\linewidth]{figures/pie_combined_50.png}}
%     \hfill
  
%   \caption{Performance analysis of combined prompt for different sample size(k)}
%   \label{fig:combined_pie} 
% \end{figure*}

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/pie_combined.pdf}
%     \caption{Performance analysis of combined prompt for different sample size(k)}
%     \label{fig:combined_pie}
% \end{figure*}




% \lessons{Prompting with the instruction set with few-shot examples are performing similarly to few-shot prompting for the low-level program specification tasks  \saikat{What? -- How do you learn this lessos?}}

\lessons{With an integrated approach combining GIs and few-shot prompting, GPT-4o achieved a success rate of up to 78\% for $k=50$, the highest across all our experiments.}

% \lessons{The performance difference between using few-shot examples alone and integrated few-shot examples with GIs is quite subtle, with a maximum improvement of approximately 2\%.}

 

% \paragraph{Discussion on the findings of RQ1.3}

\subsection{ \textbf{ [RQ2] Can LLM repair the incorrect loop invariants} }

From our study of \textbf{RQ1}, we observed that the best-performing setup, $\mathcal{EX}_{P}$ if successful for 76\% of the problems when we generate upto 50 invariants per problem. 
% This suggests that an LLM must generate up to 50 invariants per problem to reach a 76\% likelihood of synthesizing a correct one. 
To improve efficiency and reduce the need for generating a large number of samples, an intuitive solution would be to repair incorrect invariants. Instead of generating multiple invariants from scratch, we investigate whether LLMs can repair unsuccessful invariants using feedback from the verifier. To structure this investigation, we divided \textbf{RQ2} into two sub-questions: 


\begin{itemize}
    \item \textbf{[RQ2.1]} Can LLM repair the unsuccessful invariants by analyzing the cause of failure?
    \item \textbf{[RQ2.2]} Does providing more detailed error information assist in repairing invariants?
    % \item \textbf{[RQ2.3]} Why repaired invariants are failing?
\end{itemize}


\subsubsection{[RQ2.1]} Can LLM repair the unsuccessful invariants by analyzing the cause of failure?

\motivation 
% Our observation of LLM's generation of invariants indicates that LLM takes up to 30 to 50 samples to verify a problem \saikat{This sentence does not sound right, is this true?}. For a dataset of 210 problems, currently, we are in requirement \saikat{what do you mean by we are in requirement?} of generating 210*50 (equivalently 10500) invariants to test those problems, which is comparatively a bigger number, while we need only 210 invariants to verify the problems. To cope with this issue, our study tried to examine the correctness ability of LLMs from an unsuccessful invariant to a successful invariant. To aid this, the verifier feedback corresponding to the unsatisfying invariant can play a good role. \saikat{I kind of understand what you are trying to say here. If I am not mistaken, you are trying to say "instead of generating n different solution, what if we tried repairing 1 solution?". If my assumption is correct, this paragraph is sort of ambiguous. }

Upon observing a large number of failed invariants, we investigated the underlying cause of the error by analyzing the error messages generated from the verifier.

-  \saikat{What do you mean by key insight? What are the insights? I think the 2 sentences above should be removed - updated}
The feedback from the verifier highlights the specific cause of the error and offers a detailed message describing the issue. For example, one example feedback is: "{\texttt{ \{cause: Exception\}, \{details: Expected and generated invariant function names do not match; use ...\} }}", clearly indicating the cause of the error and providing guidance for correction. This motivated us to explore the possibility of correcting the invariant based on the verifier's feedback on the incorrect invariant. This process can be instrumental in reducing the overall number of invariant generations required while maintaining verification accuracy.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/prompt_repair.drawio.pdf}
    \caption{Prompt Template to repair incorrect invariant }
    \label{fig:template_rep}
\end{figure}

\experiment
% To test the repairing capabilities of the LLMs, we selected 200 unsuccessful invariants \saikat{why 200?} from the earlier studies of 100 different problems \saikat{were these 100 problems not verified with any of the models? How did you choose these 100 and 200? This is very confusing.} and their corresponding verifier feedback. The prompt was prepared by specifying the SyGus problem\saikat{not SyGus Problem}, generated invariant, and the verifier's response caused by the failure to satisfy the verification conditions. We were consistent with the GPT-4o model for this experiment, too. 

To conduct this experiment, we instructed the LLM to generate invariants for all problems in our benchmark. Each generated invariant was subsequently tested for correctness. If an invariant was found to be incorrect, we recorded the corresponding feedback from the verifier. For every problem, we selected the first two incorrect invariants and asked the LLM to repair them using the verifier's feedback, which includes an error title and a detailed error message. We incorporated this feedback into the prompt to guide the repair requests. Figure \ref{fig:template_rep} illustrates the template of the prompt used for repairs. 

\begin{table}
    \caption{LLMs Performance in Invariant Repair Using Errors}
    \centering
    \footnotesize{
    \begin{tabular} {c|c|c|c}
    
    % \begin{tabular}{cclc}
         LLM Model&  \# Problems &   \# Attempted invariants & \%  Successful repair \bigstrut \\
         \hlineB{2}
         GPT-4o&  210&   420& 6\% \bigstrut \\ 
         Mistral-Large&  210&   420& 4\% \bigstrut \\ 
         \hlineB{2}
    \end{tabular}   
    }
    \label{tab:llmRepairInv}
\end{table}


\resultsec
% Among the 200 unsuccessful invariants, on average, five invariants were successfully modified to verify the corresponding problems with three iterative attempts.  \saikat{you need to show more on these results. What do you mean by on average, on average between what?}

Table \ref{tab:llmRepairInv} presents the results of our study evaluating the effectiveness of LLMs in repairing incorrect invariants. Out of 420 generated incorrect invariants (the first 2 incorrect invariants for each of the 210 problems), GPT-4 successfully repaired only 6\%, while Mistral-large achieved a slightly lower success rate of 4\%. These results demonstrate that, even with verifier feedback, both models struggled to consistently transform incorrect invariants into correct ones. The low success rates suggest that LLMs may have difficulty understanding and applying verifier feedback effectively or generalizing corrections across diverse error types. Given this inefficiency, relying exclusively on repair-based approaches may not yet be a viable alternative to generating multiple independent invariants. 
\saikat{Does that mean all 420 initial generations that you tried to repair are all incorrect? That doesn't seem right.
}

\todo {reply: We have selected 420 incorrect invariants to repair, not the first 420 invariants. 
Texts updated to make it clearer}

% \lessons{The loop invariants verification failure cause is not helpful to repair the invariants with LLMs \saikat{Again, there is no evidence supporting this. }}
% \lessons{Only the cause of failure is not sufficient to guide the LLM to repair the invariants \saikat{this claim is completely unsubstantiated}}

% \lessons{With a maximum of 6\% success in invariant repair using the verifier feedback, }

\subsubsection{RQ2.2} Does providing more detailed error information assist in repairing invariants?

\motivation
% From the above study, we dug into the dipper \saikat{?} to find more detailed information from the verifier. Using the verifier log information, we revealed that, for each of the verifying conditions, as mentioned in the section \ref{sygus-conditions}, the verifier internally prepares a model to check for which values of the participating variables the invariant is failing to become true\saikat{A reader would have no background on what a model is, and why is this important}. Exacting the model facilitated us to provide the LLM with more detailed information about the failure of the invariant. So, we were interested in examining the ability of LLMs to update the invariants based on the failure model information.

To investigate the lower success rate of LLMs observed in \textbf{RQ2.1}, we assessed whether providing more detailed information about an incorrect verification could enhance the model's ability to transform an invariant into a correct one. The feedback and log analysis from the verifier offer deeper insights into the verification process. For example, as shown in Table \ref{tab: similarity}, a function $preF$ —operates on specific variables. During verification, the verifier tests these variables across a wide range of values. When verification fails, the verifier supplies feedback that includes the specific variable values that contributed to the failure. Our objective is to determine whether incorporating these variable values into the repair prompt can assist the LLM in generating more accurate corrections.

\begin{table}
    \caption{LLMs Performance in Invariant Repair Using Errors leading Values}
    \centering
    \footnotesize{
    \begin{tabular} {c|c|c|c}
    
    % \begin{tabular}{cclc}
         LLM Model&  \# Problems &   \# Attempted invariants & \%  Successful repair \bigstrut \\
         \hlineB{2}
         GPT-4o&  210&   420& 16\% \bigstrut \\ 
         Mistral-Large&  210&   420& 7\% \bigstrut \\ 
         \hlineB{2}
    \end{tabular}   
    }
    \label{tab:llmRepairInvValues}
\end{table}

\experiment
% We extracted the verifying conditions that failed verification, along with the associated variable values, by analyzing the feedback and error logs of the verifier.
Whenever an invariant fails to verify, the verifier provides us feedback on which verification condition failed and a variable value assignment, for which the condition failed (\ie counterexample). 
The prompt used in \textbf{RQ2.1} was modified to explicitly specify the unsatisfactory verification conditions and the corresponding counterexample that contributed to the verification failure. To ensure consistency, we maintained the same experimental setup as in \textbf{RQ2.1}. Figure \ref{fig: repair_steps} demonstrates an example prompt structured as a chat query for the LLM.

\resultsec
Table \ref{tab:llmRepairInvValues} presents the results of our experiment. When provided with detailed error information, GPT-4 successfully repaired 16\% of the incorrect invariants, while Mistral-large achieved a success rate of 7\%. Both models demonstrated improvement compared to the baseline setup in \textbf{RQ2.1}, where they exhibited significantly lower success rates. These results indicate that explicit details about unsatisfied conditions and the variable values causing verification failures enable LLMs to make more informed corrections. However, despite this improvement, the overall success rates remain relatively low, suggesting that LLMs still struggle to fully understand and effectively utilize verifier feedback for invariant repair. 

% \lessons{
% LLM can repair the failed invariants using the cause of failure \saikat{No evidence?}
% }

% \lessons{ The success ratio is not very significant to consider repairing with the current setup \saikat{what significance test did you do?}}

\lessons{Although achieving a relatively low success rate of up to 16\%, LLMs perform marginally better at repairing incorrect invariants when provided with the exact variable values that caused the verification errors}

% \subsubsection{[RQ2.3]} Why repaired invariants are failing?

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/casestudy.pdf}
    \caption{Invariant repairing with LLM}
    \label{fig: repair_steps}
\end{figure*}

\textbf{\paragraph{Observation:} LLM Repairing process with detailed Information} 

To understand the LLM's invariant repair process, we closely examined a specific case, illustrated in Figure \ref{fig: repair_steps}. Our observations reveal that when the LLM is provided with detailed information for repairing an invariant, it attempts to address the specific failure case mentioned in the prompt during its first revision. For example, in the case shown in Figure \ref{fig: repair_steps}, the invariant (I1) failed for the case \textit{n = -1}. The LLM responded by repairing the invariant and producing a new version (I2). While I2 successfully passed the case \textit{n = -1}, it failed for a new case, \textit{n = -2}. A subsequent repair request led the LLM to generate another invariant (I3), which satisfied \textit{n = -2} but failed for a different case. This iterative process continued, with the LLM eventually recreating earlier invariants, such as I1, and repairing them again into I2, creating a loop of repeated, incorrect invariants. This behavior suggests that while LLMs can make localized fixes based on specific failures, they often lack a global understanding of the invariant space, highlighting the need for strategies that promote generalization rather than reactive generation.


% Future work may focus on breaking this repetitive cycle to improve the robustness of LLMs in loop invariant repair tasks.


 
\saikat{After reading this section, a reader is not convinced if repair is a worth it investment. If repair should be done.}

% \lessons{LLMs are too strict in repairing the invariants with given case}
% \lessons{LLMs are generating the same set of invariants recurrently \saikat{See 4-27, we may need to move this whole thing to section 5}}

% \saikat{This whole study is anecdotal, lacking scientific rigot. While this is interesting, any finding from this study cannot be a throry, it is merely a conjecture.} 

==> body/6.limitation.tex <==
\section{Limitation \& Threats to Validity}

\subsection{Limitation}
% The study has several limitations. First, the study is limited to the sygus programming problems. The findings may not be generalized to other programming languages. Second, the study is limited to the use of the OpenAI, Mistral-ai, and Llama LLM models. The findings may not be generalized to other LLMs. Additionally, the study is limited to the use of the few-shot learning approach. The findings may not be generalized to other machine-learning approaches. We have limitations of computational resources that restrict us from using the larger models of open-source LLMs. Third, the study is limited to the use of the Z3 solver for invariant verification. The findings may not be generalized to other SMT solvers. 

This study has several limitations that may affect the generalization of its findings. First, our evaluation is confined to SMT-style loop specification benchmarks, which may not represent the broader spectrum of programming tasks or languages. Second, we limit our analysis to a subset of prominent LLMs- OpenAI's GPT models, Mistral, and LLaMA. Due to computational limitations, we were unable to evaluate larger variants of LLaMA models, and the performance observed on our setup may not reflect the models’ full potential. Consequently, our conclusions may not extend to other LLM architectures or proprietary systems. Third, our prompting strategy is based solely on few-shot learning; we do not explore other paradigms such as fine-tuning or in-context learning approaches. Finally, we use the Z3 SMT solver as the sole verifier for invariant correctness, and our results may not directly translate to other verification backends.

\subsection{Threats to Validity}

The validity of the study can be threatened by several factors. First, the validity of the study can be compromised by the quality of the problem scenario. In this study, we examined the solvable problems and the invariants that are feasible to generate. The quality of the generated invariants can be influenced by the quality of the prompt, the quality of the LLM, and the quality of the few-shot examples. Second, for the open-source LLMs we examined, the processing unit we used may have adversely affected the performance of the LLMs. We observed that open-source LLMs are way better with their larger models as well as with their interactive chat UIs. Third, the validity of the study can be threatened by the quality of the Z3 solver. We didn't question the quality of the Z3 solver that comes with the solution prepared by \cite{padhi2016data}. Fourth, the LLM-generated responses are natural texts; in many cases, those are not syntactically correct or contain imbalanced parentheses. We have to manually correct those before feeding them to the Z3 solver. This manual correction can be a threat to the validity of the study. Further, the non-deterministic generative nature of the LLMs keeps the door open to question the reproducibility of the same set of outputs.    

==> body/data.tex <==
\section{Data}
We utilized the Loop Invariant Synthesis benchmark dataset curated by Padhi~\etal~ \cite{padhi2016data}, for this study. This dataset consists of 940 problems formatted in SMT~\cite{alur2013syntax}. The dataset was further analyzed by Chakraborty~\etal~\cite{chakraborty2023ranking}, who identified 429 problems with at least one invariant satisfying all verification conditions. From these 429 problems, we randomly selected 210 problems to evaluate different models. To determine the appropriate sample size for our study, we applied the sample size calculation rule proposed by Uddin~\etal~ \cite{uddin2022empirical}, We determined the sample size using a 98\% confidence level, a 5\% margin of error, and an assumed population proportion of 75\%.

